Leveraging Domain Features for Detecting Adversarial Attacks Against Deep Speech Recognition in Noise

In recent years, significant progress has been made in deep model-based automatic speech recognition (ASR), leading to its widespread deployment in the real world. At the same time, adversarial attacks against deep ASR systems are highly successful. Various methods have been proposed to defend ASR systems from these attacks. However, existing classification based methods focus on the design of deep learning models while lacking exploration of domain specific features. This work leverages filter bank-based features to better capture the characteristics of attacks for improved detection. Furthermore, the paper analyses the potentials of using speech and non-speech parts separately in detecting adversarial attacks. In the end, considering adverse environments where ASR systems may be deployed, we study the impact of acoustic noise of various types and signal-to-noise ratios. Extensive experiments show that the inverse filter bank features generally perform better in both clean and noisy environments, the detection is effective using either speech or non-speech part, and the acoustic noise can largely degrade the detection performance.

==> exclude/asru_guides.tex <==
TYPE:

Face: To achieve the best viewing experience for the review process and conference proceedings, we strongly encourage authors to use Times-Roman or Computer Modern fonts. If a font face is used that is not recognized by the submission system, your submission will not be reproduced correctly.

Size: Use a font size that is no smaller than 9 points throughout the paper, including figure captions. In 9-point type font, capital letters are 2 mm high. For 9-point type font, there should be no more than 3.2 lines/cm (8 lines/inch) vertically. This is a minimum spacing; 2.75 lines/cm (7 lines/inch) will make the submission much more readable. Larger type sizes require correspondingly larger vertical spacing.

TITLE: The paper title must appear in boldface letters and should be in ALL CAPITALS. Do not use LaTeX math notation ($x_y$) in the title; the title must be representable in the Unicode character set. Also try to avoid uncommon acronyms in the title.

AUTHOR LIST: The authors' name(s) and affiliation(s) appear below the title in capital and lower case letters. Submissions with multiple authors and affiliations may require two or more lines for this information. The order of the authors on the document should exactly match in number and order the authors typed into the online submission form.

ABSTRACT: Each paper should contain an abstract of approximately 100 to 150 words that appears at the beginning of the document. Use the same text that is submitted electronically along with the author contact information.

INDEX TERMS (KEYWORDS): Enter up to 5 keywords separated by commas.

BODY: Major headings appear in boldface CAPITAL letters, centered in the column. Subheadings appear in capital and lower case, either underlined or in boldface. They start at the left margin of the column on a separate line. Sub-subheadings are discouraged, but if they must be used, they should appear in capital and lower case, and start at the left margin on a separate line. They may be underlined or in italics.

REFERENCES: List and number all references at the end of the document. The references can be numbered in alphabetical order or in order of appearance in the paper. When referring to them in the text, type the corresponding reference number in square brackets as shown at the end of this sentence [1]. The end of the document should include a list of references containing information similar to the following example:

[1] D. E. Ingalls, "Image Processing for Experts," IEEE Trans. ASSP, vol. ASSP-36, pp. 1932-1948, 1988.

ILLUSTRATIONS & COLOR: Illustrations must appear within the designated margins. They may span the two columns. If possible, position illustrations at the top of columns, rather than in the middle or at the bottom. Caption and number every illustration. All halftone illustrations must be clear in black and white. Since the printed proceedings will be produced in black and white, be sure that your images are acceptable when printed in black and white (the electronic and IEEE Xplore proceedings will retain the colors in your document).

PAGE NUMBERS: Do not put page numbers on your document. Appropriate page numbers will be added to accepted papers when the conference proceedings are assembled.

==> exclude/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}



\end{enumerate}

==> figures/cepstral_coeffients.tex <==



\begin{figure} % TODO: choose short2short examples instead, plot the entire sample not only the blocks.
    \centering
    \foreach \transName in {lfcc,mfcc,imfcc,gfcc,igfcc} {
      \begin{subfigure}[b]{\subfigurewidth}
        \includegraphics[width=\textwidth]{transformations/\transName_adv-long2short-000103.block4}
        \caption{\reprname{\transName}}\label{fig:filterbank_coef_\transName}
      \end{subfigure}
    }
    \caption{Cepstral coefficients}\label{fig:cepstral_coefficients}
\end{figure}



==> figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_a/table.tex <==
\begin{table}
  \caption{merge ab test ab model ab ab test a}
  \label{tab:merge_ab_test_ab_model_ab_ab_test_a}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.944 \pm 0.006$ &               $0.94 \pm 0.011$ &           $0.929 \pm 0.019$ &                                  $0.942 \pm 0.007$ \\
  igfcc &             $0.985 \pm 0.002$ &              $0.983 \pm 0.005$ &           $0.983 \pm 0.005$ &                                  $0.985 \pm 0.002$ \\
  imfcc &    $\mathbf{0.989 \pm 0.002}$ &     $\mathbf{0.986 \pm 0.005}$ &  $\mathbf{0.989 \pm 0.003}$ &                         $\mathbf{0.989 \pm 0.002}$ \\
  lfcc  &             $0.976 \pm 0.001$ &              $0.969 \pm 0.008$ &           $0.976 \pm 0.008$ &                                  $0.976 \pm 0.001$ \\
  mfcc  &             $0.965 \pm 0.001$ &               $0.957 \pm 0.01$ &            $0.96 \pm 0.012$ &                                  $0.964 \pm 0.002$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_a_b/table.tex <==
\begin{table}
  \caption{merge ab test ab model ab ab test a b}
  \label{tab:merge_ab_test_ab_model_ab_ab_test_a_b}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.95 \pm 0.006$ &              $0.946 \pm 0.011$ &           $0.938 \pm 0.016$ &                                  $0.948 \pm 0.006$ \\
  igfcc &             $0.986 \pm 0.001$ &              $0.986 \pm 0.004$ &           $0.983 \pm 0.005$ &                                  $0.986 \pm 0.001$ \\
  imfcc &    $\mathbf{0.989 \pm 0.002}$ &     $\mathbf{0.987 \pm 0.004}$ &  $\mathbf{0.989 \pm 0.004}$ &                         $\mathbf{0.989 \pm 0.002}$ \\
  lfcc  &             $0.979 \pm 0.001$ &              $0.974 \pm 0.007$ &           $0.977 \pm 0.007$ &                                  $0.979 \pm 0.001$ \\
  mfcc  &             $0.966 \pm 0.001$ &              $0.961 \pm 0.009$ &           $0.962 \pm 0.009$ &                                  $0.966 \pm 0.001$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_b/table.tex <==
\begin{table}
  \caption{merge ab test ab model ab ab test b}
  \label{tab:merge_ab_test_ab_model_ab_ab_test_b}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.972 \pm 0.012$ &              $0.969 \pm 0.016$ &           $0.972 \pm 0.012$ &                                  $0.972 \pm 0.012$ \\
  igfcc &    $\mathbf{0.991 \pm 0.005}$ &     $\mathbf{0.998 \pm 0.002}$ &           $0.982 \pm 0.009$ &                          $\mathbf{0.99 \pm 0.005}$ \\
  imfcc &    $\mathbf{0.991 \pm 0.007}$ &              $0.992 \pm 0.005$ &  $\mathbf{0.988 \pm 0.011}$ &                          $\mathbf{0.99 \pm 0.007}$ \\
  lfcc  &             $0.988 \pm 0.003$ &              $0.993 \pm 0.004$ &           $0.982 \pm 0.005$ &                                  $0.988 \pm 0.003$ \\
  mfcc  &             $0.974 \pm 0.004$ &              $0.976 \pm 0.008$ &           $0.969 \pm 0.006$ &                                  $0.974 \pm 0.004$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/table.tex <==
\begin{tabular}{lllllll}
\toprule
                          & transformation & \rotatebox{0}{gfcc} & \rotatebox{0}{igfcc} & \rotatebox{0}{imfcc} & \rotatebox{0}{lfcc} & \rotatebox{0}{mfcc} \\
\midrule
merge\_ab\_test\_ab\_model\_ab\_ab & test\_a &   $0.942 \pm 0.007$ &    $0.985 \pm 0.002$ &    $0.989 \pm 0.002$ &   $0.976 \pm 0.001$ &   $0.964 \pm 0.002$ \\
                          & test\_a\_b &   $0.948 \pm 0.006$ &    $0.986 \pm 0.001$ &    $0.989 \pm 0.002$ &   $0.979 \pm 0.001$ &   $0.966 \pm 0.001$ \\
                          & test\_b &   $0.972 \pm 0.012$ &     $0.99 \pm 0.005$ &     $0.99 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.974 \pm 0.004$ \\
truncated\_a\_model\_a\_a & test\_a &    $0.915 \pm 0.02$ &    $0.981 \pm 0.003$ &     $0.98 \pm 0.003$ &   $0.961 \pm 0.003$ &   $0.941 \pm 0.013$ \\
                          & test\_b &    $0.694 \pm 0.04$ &    $0.932 \pm 0.012$ &     $0.946 \pm 0.01$ &   $0.692 \pm 0.127$ &   $0.576 \pm 0.072$ \\
truncated\_a\_silence\_model\_silence\_silence & test\_silence &   $0.965 \pm 0.014$ &    $0.995 \pm 0.004$ &    $0.993 \pm 0.006$ &   $0.988 \pm 0.006$ &    $0.97 \pm 0.016$ \\
                          & test\_speech &   $0.661 \pm 0.058$ &    $0.851 \pm 0.071$ &     $0.823 \pm 0.06$ &   $0.746 \pm 0.042$ &   $0.724 \pm 0.074$ \\
truncated\_a\_speech\_model\_speech\_speech & test\_silence &   $0.863 \pm 0.033$ &    $0.988 \pm 0.011$ &    $0.987 \pm 0.009$ &    $0.948 \pm 0.02$ &   $0.937 \pm 0.017$ \\
                          & test\_speech &   $0.679 \pm 0.036$ &    $0.945 \pm 0.018$ &    $0.944 \pm 0.021$ &   $0.886 \pm 0.028$ &   $0.833 \pm 0.051$ \\
truncated\_b\_model\_b\_b & test\_a &   $0.528 \pm 0.011$ &    $0.676 \pm 0.034$ &    $0.672 \pm 0.091$ &   $0.625 \pm 0.057$ &   $0.527 \pm 0.015$ \\
                          & test\_b &   $0.982 \pm 0.004$ &    $0.991 \pm 0.005$ &    $0.991 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.983 \pm 0.005$ \\
\bottomrule
\end{tabular}


==> figures/latex/1614926381/truncated_a_model_a_a/test_a/table.tex <==
\begin{table}
  \caption{truncated a model a a test a}
  \label{tab:truncated_a_model_a_a_test_a}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.917 \pm 0.024$ &              $0.898 \pm 0.044$ &           $0.903 \pm 0.016$ &                                   $0.915 \pm 0.02$ \\
  igfcc &    $\mathbf{0.982 \pm 0.005}$ &     $\mathbf{0.976 \pm 0.018}$ &             $0.98 \pm 0.01$ &                         $\mathbf{0.981 \pm 0.003}$ \\
  imfcc &              $0.98 \pm 0.003$ &               $0.969 \pm 0.01$ &   $\mathbf{0.982 \pm 0.01}$ &                                   $0.98 \pm 0.003$ \\
  lfcc  &             $0.963 \pm 0.003$ &               $0.957 \pm 0.02$ &           $0.952 \pm 0.016$ &                                  $0.961 \pm 0.003$ \\
  mfcc  &             $0.944 \pm 0.014$ &              $0.941 \pm 0.034$ &           $0.922 \pm 0.023$ &                                  $0.941 \pm 0.013$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_a_model_a_a/test_b/table.tex <==
\begin{table}
  \caption{truncated a model a a test b}
  \label{tab:truncated_a_model_a_a_test_b}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.706 \pm 0.037$ &              $0.841 \pm 0.054$ &            $0.472 \pm 0.11$ &                                   $0.694 \pm 0.04$ \\
  igfcc &             $0.936 \pm 0.012$ &     $\mathbf{0.999 \pm 0.002}$ &           $0.866 \pm 0.025$ &                                  $0.932 \pm 0.012$ \\
  imfcc &     $\mathbf{0.949 \pm 0.01}$ &              $0.996 \pm 0.003$ &   $\mathbf{0.895 \pm 0.02}$ &                          $\mathbf{0.946 \pm 0.01}$ \\
  lfcc  &             $0.708 \pm 0.121$ &              $0.988 \pm 0.012$ &           $0.387 \pm 0.255$ &                                  $0.692 \pm 0.127$ \\
  mfcc  &             $0.596 \pm 0.069$ &              $0.702 \pm 0.177$ &           $0.194 \pm 0.147$ &                                  $0.576 \pm 0.072$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_a_silence_model_silence_silence/test_silence/table.tex <==
\begin{table}
  \caption{truncated a silence model silence silence test silence}
  \label{tab:truncated_a_silence_model_silence_silence_test_silence}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.967 \pm 0.017$ &              $0.925 \pm 0.052$ &           $0.962 \pm 0.022$ &                                  $0.965 \pm 0.014$ \\
  igfcc &    $\mathbf{0.995 \pm 0.003}$ &     $\mathbf{0.989 \pm 0.011}$ &  $\mathbf{0.994 \pm 0.009}$ &                         $\mathbf{0.995 \pm 0.004}$ \\
  imfcc &             $0.994 \pm 0.004$ &              $0.987 \pm 0.004$ &           $0.991 \pm 0.012$ &                                  $0.993 \pm 0.006$ \\
  lfcc  &             $0.991 \pm 0.006$ &              $0.983 \pm 0.019$ &           $0.983 \pm 0.007$ &                                  $0.988 \pm 0.006$ \\
  mfcc  &             $0.974 \pm 0.016$ &              $0.951 \pm 0.036$ &            $0.96 \pm 0.016$ &                                   $0.97 \pm 0.016$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_a_silence_model_silence_silence/test_speech/table.tex <==
\begin{table}
  \caption{truncated a silence model silence silence test speech}
  \label{tab:truncated_a_silence_model_silence_silence_test_speech}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.775 \pm 0.038$ &              $0.555 \pm 0.124$ &           $0.441 \pm 0.156$ &                                  $0.661 \pm 0.058$ \\
  igfcc &    $\mathbf{0.914 \pm 0.031}$ &              $0.882 \pm 0.063$ &   $\mathbf{0.732 \pm 0.15}$ &                         $\mathbf{0.851 \pm 0.071}$ \\
  imfcc &              $0.904 \pm 0.03$ &      $\mathbf{0.901 \pm 0.04}$ &            $0.67 \pm 0.127$ &                                   $0.823 \pm 0.06$ \\
  lfcc  &             $0.868 \pm 0.018$ &              $0.853 \pm 0.045$ &           $0.519 \pm 0.088$ &                                  $0.746 \pm 0.042$ \\
  mfcc  &             $0.825 \pm 0.019$ &               $0.678 \pm 0.08$ &           $0.534 \pm 0.189$ &                                  $0.724 \pm 0.074$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_a_speech_model_speech_speech/test_silence/table.tex <==
\begin{table}
  \caption{truncated a speech model speech speech test silence}
  \label{tab:truncated_a_speech_model_speech_speech_test_silence}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.86 \pm 0.055$ &               $0.722 \pm 0.12$ &           $0.869 \pm 0.086$ &                                  $0.863 \pm 0.033$ \\
  igfcc &             $0.984 \pm 0.016$ &              $0.951 \pm 0.052$ &  $\mathbf{0.998 \pm 0.005}$ &                         $\mathbf{0.988 \pm 0.011}$ \\
  imfcc &     $\mathbf{0.987 \pm 0.01}$ &     $\mathbf{0.966 \pm 0.033}$ &           $0.987 \pm 0.013$ &                                  $0.987 \pm 0.009$ \\
  lfcc  &             $0.935 \pm 0.036$ &              $0.824 \pm 0.099$ &           $0.976 \pm 0.024$ &                                   $0.948 \pm 0.02$ \\
  mfcc  &             $0.923 \pm 0.033$ &              $0.807 \pm 0.086$ &           $0.966 \pm 0.027$ &                                  $0.937 \pm 0.017$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_a_speech_model_speech_speech/test_speech/table.tex <==
\begin{table}
  \caption{truncated a speech model speech speech test speech}
  \label{tab:truncated_a_speech_model_speech_speech_test_speech}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.801 \pm 0.018$ &               $0.64 \pm 0.124$ &           $0.446 \pm 0.118$ &                                  $0.679 \pm 0.036$ \\
  igfcc &     $\mathbf{0.965 \pm 0.01}$ &              $0.941 \pm 0.042$ &  $\mathbf{0.907 \pm 0.035}$ &                         $\mathbf{0.945 \pm 0.018}$ \\
  imfcc &             $0.964 \pm 0.014$ &     $\mathbf{0.943 \pm 0.029}$ &           $0.904 \pm 0.037$ &                                  $0.944 \pm 0.021$ \\
  lfcc  &             $0.914 \pm 0.015$ &              $0.809 \pm 0.038$ &           $0.832 \pm 0.065$ &                                  $0.886 \pm 0.028$ \\
  mfcc  &             $0.886 \pm 0.025$ &              $0.776 \pm 0.074$ &           $0.731 \pm 0.108$ &                                  $0.833 \pm 0.051$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_b_model_b_b/test_a/table.tex <==
\begin{table}
  \caption{truncated b model b b test a}
  \label{tab:truncated_b_model_b_b_test_a}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.609 \pm 0.021$ &              $0.689 \pm 0.089$ &           $0.081 \pm 0.021$ &                                  $0.528 \pm 0.011$ \\
  igfcc &    $\mathbf{0.718 \pm 0.023}$ &     $\mathbf{0.805 \pm 0.098}$ &  $\mathbf{0.437 \pm 0.125}$ &                         $\mathbf{0.676 \pm 0.034}$ \\
  imfcc &             $0.715 \pm 0.071$ &               $0.789 \pm 0.04$ &           $0.424 \pm 0.225$ &                                  $0.672 \pm 0.091$ \\
  lfcc  &              $0.684 \pm 0.04$ &              $0.794 \pm 0.078$ &           $0.307 \pm 0.145$ &                                  $0.625 \pm 0.057$ \\
  mfcc  &              $0.61 \pm 0.022$ &              $0.723 \pm 0.062$ &           $0.077 \pm 0.041$ &                                  $0.527 \pm 0.015$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1614926381/truncated_b_model_b_b/test_b/table.tex <==
\begin{table}
  \caption{truncated b model b b test b}
  \label{tab:truncated_b_model_b_b_test_b}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.983 \pm 0.004$ &              $0.984 \pm 0.007$ &           $0.979 \pm 0.009$ &                                  $0.982 \pm 0.004$ \\
  igfcc &             $0.991 \pm 0.005$ &              $0.993 \pm 0.005$ &  $\mathbf{0.989 \pm 0.008}$ &                         $\mathbf{0.991 \pm 0.005}$ \\
  imfcc &    $\mathbf{0.992 \pm 0.007}$ &     $\mathbf{0.994 \pm 0.004}$ &           $0.988 \pm 0.011$ &                         $\mathbf{0.991 \pm 0.007}$ \\
  lfcc  &             $0.988 \pm 0.003$ &               $0.99 \pm 0.005$ &           $0.984 \pm 0.008$ &                                  $0.988 \pm 0.003$ \\
  mfcc  &             $0.983 \pm 0.005$ &               $0.985 \pm 0.01$ &           $0.979 \pm 0.012$ &                                  $0.983 \pm 0.005$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_0db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 0db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &    $\mathbf{0.783 \pm 0.094}$ &              $0.173 \pm 0.074$ &           $0.336 \pm 0.127$ &                                  $0.579 \pm 0.024$ \\
  igfcc &             $0.724 \pm 0.052$ &               $0.16 \pm 0.022$ &   $\mathbf{0.55 \pm 0.053}$ &                                  $0.644 \pm 0.017$ \\
  imfcc &              $0.78 \pm 0.052$ &     $\mathbf{0.191 \pm 0.035}$ &           $0.497 \pm 0.065$ &                         $\mathbf{0.651 \pm 0.017}$ \\
  lfcc  &             $0.755 \pm 0.071$ &               $0.17 \pm 0.033$ &           $0.489 \pm 0.096$ &                                   $0.634 \pm 0.03$ \\
  mfcc  &              $0.76 \pm 0.037$ &               $0.14 \pm 0.013$ &           $0.376 \pm 0.072$ &                                  $0.585 \pm 0.019$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_0db_pcafeter_snr_5db_pcafeter_snr_10db_pcafeter_snr_15db_pcafeter_snr_20db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 0db pcafeter snr 5db pcafeter snr 10db pcafeter snr 15db pcafeter snr 20db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_0db_pcafeter_snr_5db_pcafeter_snr_10db_pcafeter_snr_15db_pcafeter_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.832 \pm 0.06$ &              $0.285 \pm 0.113$ &            $0.532 \pm 0.09$ &                                  $0.695 \pm 0.019$ \\
  igfcc &             $0.852 \pm 0.027$ &              $0.328 \pm 0.043$ &  $\mathbf{0.749 \pm 0.035}$ &                         $\mathbf{0.805 \pm 0.009}$ \\
  imfcc &    $\mathbf{0.878 \pm 0.023}$ &      $\mathbf{0.377 \pm 0.05}$ &           $0.708 \pm 0.057$ &                                  $0.801 \pm 0.016$ \\
  lfcc  &              $0.864 \pm 0.04$ &              $0.346 \pm 0.073$ &            $0.66 \pm 0.041$ &                                  $0.771 \pm 0.016$ \\
  mfcc  &             $0.828 \pm 0.039$ &              $0.262 \pm 0.049$ &           $0.572 \pm 0.065$ &                                  $0.711 \pm 0.026$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_10db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 10db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.826 \pm 0.059$ &              $0.269 \pm 0.085$ &           $0.525 \pm 0.126$ &                                  $0.689 \pm 0.031$ \\
  igfcc &             $0.868 \pm 0.025$ &               $0.36 \pm 0.051$ &  $\mathbf{0.758 \pm 0.033}$ &                         $\mathbf{0.818 \pm 0.016}$ \\
  imfcc &     $\mathbf{0.885 \pm 0.02}$ &     $\mathbf{0.393 \pm 0.044}$ &            $0.71 \pm 0.083$ &                                  $0.805 \pm 0.032$ \\
  lfcc  &             $0.876 \pm 0.039$ &               $0.379 \pm 0.09$ &           $0.675 \pm 0.043$ &                                  $0.785 \pm 0.027$ \\
  mfcc  &             $0.829 \pm 0.042$ &              $0.263 \pm 0.053$ &            $0.56 \pm 0.084$ &                                  $0.707 \pm 0.033$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_15db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 15db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.862 \pm 0.044$ &              $0.353 \pm 0.128$ &            $0.638 \pm 0.04$ &                                   $0.76 \pm 0.022$ \\
  igfcc &              $0.92 \pm 0.016$ &              $0.508 \pm 0.054$ &  $\mathbf{0.871 \pm 0.033}$ &                         $\mathbf{0.898 \pm 0.017}$ \\
  imfcc &     $\mathbf{0.931 \pm 0.01}$ &     $\mathbf{0.554 \pm 0.055}$ &           $0.834 \pm 0.056$ &                                  $0.887 \pm 0.022$ \\
  lfcc  &             $0.919 \pm 0.026$ &              $0.519 \pm 0.101$ &           $0.754 \pm 0.019$ &                                  $0.844 \pm 0.011$ \\
  mfcc  &              $0.868 \pm 0.04$ &              $0.362 \pm 0.087$ &           $0.684 \pm 0.078$ &                                  $0.784 \pm 0.041$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_20db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 20db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.889 \pm 0.033$ &              $0.421 \pm 0.117$ &           $0.725 \pm 0.075$ &                                  $0.814 \pm 0.032$ \\
  igfcc &             $0.955 \pm 0.012$ &               $0.67 \pm 0.074$ &   $\mathbf{0.92 \pm 0.022}$ &                         $\mathbf{0.939 \pm 0.007}$ \\
  imfcc &     $\mathbf{0.96 \pm 0.009}$ &     $\mathbf{0.706 \pm 0.068}$ &           $0.894 \pm 0.038$ &                                   $0.93 \pm 0.017$ \\
  lfcc  &             $0.951 \pm 0.013$ &              $0.667 \pm 0.078$ &           $0.818 \pm 0.035$ &                                   $0.89 \pm 0.017$ \\
  mfcc  &             $0.904 \pm 0.041$ &               $0.482 \pm 0.13$ &           $0.787 \pm 0.046$ &                                  $0.851 \pm 0.022$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_5db/table.tex <==
\begin{table}
  \caption{noises all snr to pcafeter model all noise snr all noise snr test pcafeter snr 5db}
  \label{tab:noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr_test_pcafeter_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.801 \pm 0.077$ &              $0.217 \pm 0.077$ &           $0.434 \pm 0.133$ &                                  $0.634 \pm 0.023$ \\
  igfcc &             $0.794 \pm 0.035$ &              $0.232 \pm 0.028$ &  $\mathbf{0.644 \pm 0.063}$ &                                  $0.726 \pm 0.018$ \\
  imfcc &    $\mathbf{0.834 \pm 0.038}$ &     $\mathbf{0.278 \pm 0.045}$ &           $0.607 \pm 0.086$ &                         $\mathbf{0.731 \pm 0.027}$ \\
  lfcc  &             $0.818 \pm 0.056$ &              $0.251 \pm 0.057$ &           $0.562 \pm 0.045$ &                                  $0.701 \pm 0.014$ \\
  mfcc  &             $0.782 \pm 0.045$ &              $0.177 \pm 0.029$ &           $0.441 \pm 0.068$ &                                  $0.627 \pm 0.023$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618398903/table.tex <==
\begin{tabular}{lllllll}
\toprule
                          & transformation & \rotatebox{0}{gfcc} & \rotatebox{0}{igfcc} & \rotatebox{0}{imfcc} & \rotatebox{0}{lfcc} & \rotatebox{0}{mfcc} \\
\midrule
merge\_ab\_test\_ab\_model\_ab\_ab & test\_a &   $0.942 \pm 0.007$ &    $0.985 \pm 0.002$ &    $0.989 \pm 0.002$ &   $0.976 \pm 0.001$ &   $0.964 \pm 0.002$ \\
                          & test\_a\_b &   $0.948 \pm 0.006$ &    $0.986 \pm 0.001$ &    $0.989 \pm 0.002$ &   $0.979 \pm 0.001$ &   $0.966 \pm 0.001$ \\
                          & test\_b &   $0.972 \pm 0.012$ &     $0.99 \pm 0.005$ &     $0.99 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.974 \pm 0.004$ \\
noises\_all\_snr\_to\_pcafeter\_model\_all\_noise\_snr\_all\_noise\_snr & test\_pcafeter\_snr\_0db &   $0.579 \pm 0.024$ &    $0.644 \pm 0.017$ &    $0.651 \pm 0.017$ &    $0.634 \pm 0.03$ &   $0.585 \pm 0.019$ \\
                          & test\_pcafeter\_snr\_0db\_pcafeter\_snr\_5db\_pcafeter\_snr\_10db\_pcafeter\_snr\_15db\_pcafeter\_snr\_20db &   $0.695 \pm 0.019$ &    $0.805 \pm 0.009$ &    $0.801 \pm 0.016$ &   $0.771 \pm 0.016$ &   $0.711 \pm 0.026$ \\
                          & test\_pcafeter\_snr\_10db &   $0.689 \pm 0.031$ &    $0.818 \pm 0.016$ &    $0.805 \pm 0.032$ &   $0.785 \pm 0.027$ &   $0.707 \pm 0.033$ \\
                          & test\_pcafeter\_snr\_15db &    $0.76 \pm 0.022$ &    $0.898 \pm 0.017$ &    $0.887 \pm 0.022$ &   $0.844 \pm 0.011$ &   $0.784 \pm 0.041$ \\
                          & test\_pcafeter\_snr\_20db &   $0.814 \pm 0.032$ &    $0.939 \pm 0.007$ &     $0.93 \pm 0.017$ &    $0.89 \pm 0.017$ &   $0.851 \pm 0.022$ \\
                          & test\_pcafeter\_snr\_5db &   $0.634 \pm 0.023$ &    $0.726 \pm 0.018$ &    $0.731 \pm 0.027$ &   $0.701 \pm 0.014$ &   $0.627 \pm 0.023$ \\
truncated\_a\_model\_a\_a & test\_a &    $0.915 \pm 0.02$ &    $0.981 \pm 0.003$ &     $0.98 \pm 0.003$ &   $0.961 \pm 0.003$ &   $0.941 \pm 0.013$ \\
                          & test\_b &    $0.694 \pm 0.04$ &    $0.932 \pm 0.012$ &     $0.946 \pm 0.01$ &   $0.692 \pm 0.127$ &   $0.576 \pm 0.072$ \\
truncated\_a\_silence\_model\_silence\_silence & test\_silence &   $0.965 \pm 0.014$ &    $0.995 \pm 0.004$ &    $0.993 \pm 0.006$ &   $0.988 \pm 0.006$ &    $0.97 \pm 0.016$ \\
                          & test\_speech &   $0.661 \pm 0.058$ &    $0.851 \pm 0.071$ &     $0.823 \pm 0.06$ &   $0.746 \pm 0.042$ &   $0.724 \pm 0.074$ \\
truncated\_a\_speech\_model\_speech\_speech & test\_silence &   $0.863 \pm 0.033$ &    $0.988 \pm 0.011$ &    $0.987 \pm 0.009$ &    $0.948 \pm 0.02$ &   $0.937 \pm 0.017$ \\
                          & test\_speech &   $0.679 \pm 0.036$ &    $0.945 \pm 0.018$ &    $0.944 \pm 0.021$ &   $0.886 \pm 0.028$ &   $0.833 \pm 0.051$ \\
truncated\_b\_model\_b\_b & test\_a &   $0.528 \pm 0.011$ &    $0.676 \pm 0.034$ &    $0.672 \pm 0.091$ &   $0.625 \pm 0.057$ &   $0.527 \pm 0.015$ \\
                          & test\_b &   $0.982 \pm 0.004$ &    $0.991 \pm 0.005$ &    $0.991 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.983 \pm 0.005$ \\
\bottomrule
\end{tabular}


==> figures/latex/1618499599/equal_mapping_bbl_morten_snr_0db_to_bbl_morten_snr_0db_model_bbl_morten_snr_0db_bbl_morten_snr_0db/test_bbl_morten_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping bbl morten snr 0db to bbl morten snr 0db model bbl morten snr 0db bbl morten snr 0db test bbl morten snr 0db}
  \label{tab:equal_mapping_bbl_morten_snr_0db_to_bbl_morten_snr_0db_model_bbl_morten_snr_0db_bbl_morten_snr_0db_test_bbl_morten_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &    $\mathbf{0.916 \pm 0.006}$ &              $0.294 \pm 0.315$ &           $0.064 \pm 0.067$ &                                  $0.528 \pm 0.029$ \\
  igfcc &             $0.911 \pm 0.012$ &              $0.471 \pm 0.081$ &   $\mathbf{0.42 \pm 0.141}$ &                         $\mathbf{0.687 \pm 0.059}$ \\
  imfcc &             $0.914 \pm 0.011$ &     $\mathbf{0.487 \pm 0.096}$ &            $0.343 \pm 0.07$ &                                  $0.654 \pm 0.027$ \\
  lfcc  &             $0.912 \pm 0.009$ &              $0.342 \pm 0.201$ &           $0.168 \pm 0.108$ &                                  $0.573 \pm 0.046$ \\
  mfcc  &              $0.912 \pm 0.01$ &              $0.146 \pm 0.205$ &            $0.08 \pm 0.113$ &                                  $0.533 \pm 0.047$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_bbl_morten_snr_10db_to_bbl_morten_snr_10db_model_bbl_morten_snr_10db_bbl_morten_snr_10db/test_bbl_morten_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping bbl morten snr 10db to bbl morten snr 10db model bbl morten snr 10db bbl morten snr 10db test bbl morten snr 10db}
  \label{tab:equal_mapping_bbl_morten_snr_10db_to_bbl_morten_snr_10db_model_bbl_morten_snr_10db_bbl_morten_snr_10db_test_bbl_morten_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.899 \pm 0.015$ &              $0.394 \pm 0.054$ &           $0.393 \pm 0.104$ &                                   $0.668 \pm 0.04$ \\
  igfcc &             $0.957 \pm 0.004$ &              $0.702 \pm 0.036$ &  $\mathbf{0.834 \pm 0.027}$ &                         $\mathbf{0.901 \pm 0.011}$ \\
  imfcc &    $\mathbf{0.962 \pm 0.005}$ &     $\mathbf{0.763 \pm 0.057}$ &           $0.777 \pm 0.037$ &                                  $0.878 \pm 0.016$ \\
  lfcc  &             $0.925 \pm 0.013$ &              $0.544 \pm 0.089$ &           $0.607 \pm 0.048$ &                                    $0.78 \pm 0.02$ \\
  mfcc  &             $0.906 \pm 0.007$ &              $0.431 \pm 0.028$ &           $0.468 \pm 0.088$ &                                  $0.706 \pm 0.038$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_bbl_morten_snr_15db_to_bbl_morten_snr_15db_model_bbl_morten_snr_15db_bbl_morten_snr_15db/test_bbl_morten_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping bbl morten snr 15db to bbl morten snr 15db model bbl morten snr 15db bbl morten snr 15db test bbl morten snr 15db}
  \label{tab:equal_mapping_bbl_morten_snr_15db_to_bbl_morten_snr_15db_model_bbl_morten_snr_15db_bbl_morten_snr_15db_test_bbl_morten_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.912 \pm 0.01$ &              $0.465 \pm 0.049$ &            $0.54 \pm 0.046$ &                                  $0.742 \pm 0.025$ \\
  igfcc &     $\mathbf{0.98 \pm 0.004}$ &     $\mathbf{0.852 \pm 0.052}$ &  $\mathbf{0.917 \pm 0.034}$ &                         $\mathbf{0.951 \pm 0.015}$ \\
  imfcc &             $0.975 \pm 0.007$ &              $0.847 \pm 0.074$ &           $0.857 \pm 0.053$ &                                  $0.921 \pm 0.024$ \\
  lfcc  &             $0.946 \pm 0.016$ &               $0.66 \pm 0.113$ &           $0.751 \pm 0.035$ &                                  $0.857 \pm 0.012$ \\
  mfcc  &              $0.92 \pm 0.015$ &              $0.509 \pm 0.061$ &           $0.653 \pm 0.023$ &                                  $0.798 \pm 0.017$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_bbl_morten_snr_20db_to_bbl_morten_snr_20db_model_bbl_morten_snr_20db_bbl_morten_snr_20db/test_bbl_morten_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping bbl morten snr 20db to bbl morten snr 20db model bbl morten snr 20db bbl morten snr 20db test bbl morten snr 20db}
  \label{tab:equal_mapping_bbl_morten_snr_20db_to_bbl_morten_snr_20db_model_bbl_morten_snr_20db_bbl_morten_snr_20db_test_bbl_morten_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.944 \pm 0.004$ &              $0.638 \pm 0.029$ &            $0.713 \pm 0.07$ &                                  $0.838 \pm 0.033$ \\
  igfcc &    $\mathbf{0.989 \pm 0.003}$ &     $\mathbf{0.951 \pm 0.038}$ &   $\mathbf{0.914 \pm 0.02}$ &                         $\mathbf{0.955 \pm 0.009}$ \\
  imfcc &             $0.986 \pm 0.002$ &              $0.915 \pm 0.041$ &           $0.913 \pm 0.021$ &                                  $0.953 \pm 0.009$ \\
  lfcc  &             $0.964 \pm 0.004$ &              $0.758 \pm 0.037$ &           $0.826 \pm 0.048$ &                                  $0.901 \pm 0.022$ \\
  mfcc  &             $0.955 \pm 0.006$ &               $0.713 \pm 0.06$ &           $0.762 \pm 0.064$ &                                   $0.867 \pm 0.03$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_bbl_morten_snr_5db_to_bbl_morten_snr_5db_model_bbl_morten_snr_5db_bbl_morten_snr_5db/test_bbl_morten_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping bbl morten snr 5db to bbl morten snr 5db model bbl morten snr 5db bbl morten snr 5db test bbl morten snr 5db}
  \label{tab:equal_mapping_bbl_morten_snr_5db_to_bbl_morten_snr_5db_model_bbl_morten_snr_5db_bbl_morten_snr_5db_test_bbl_morten_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.898 \pm 0.023$ &               $0.369 \pm 0.18$ &           $0.192 \pm 0.058$ &                                   $0.576 \pm 0.02$ \\
  igfcc &             $0.938 \pm 0.007$ &              $0.623 \pm 0.064$ &  $\mathbf{0.649 \pm 0.106}$ &                         $\mathbf{0.806 \pm 0.048}$ \\
  imfcc &    $\mathbf{0.942 \pm 0.003}$ &     $\mathbf{0.656 \pm 0.028}$ &           $0.615 \pm 0.068$ &                                  $0.793 \pm 0.032$ \\
  lfcc  &             $0.902 \pm 0.005$ &              $0.408 \pm 0.015$ &           $0.464 \pm 0.052$ &                                  $0.702 \pm 0.022$ \\
  mfcc  &              $0.91 \pm 0.009$ &              $0.435 \pm 0.053$ &             $0.276 \pm 0.1$ &                                  $0.621 \pm 0.042$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_dkitchen_snr_0db_to_dkitchen_snr_0db_model_dkitchen_snr_0db_dkitchen_snr_0db/test_dkitchen_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping dkitchen snr 0db to dkitchen snr 0db model dkitchen snr 0db dkitchen snr 0db test dkitchen snr 0db}
  \label{tab:equal_mapping_dkitchen_snr_0db_to_dkitchen_snr_0db_model_dkitchen_snr_0db_dkitchen_snr_0db_test_dkitchen_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.91 \pm 0.014$ &              $0.424 \pm 0.182$ &  $\mathbf{0.147 \pm 0.055}$ &                         $\mathbf{0.562 \pm 0.023}$ \\
  igfcc &             $0.916 \pm 0.005$ &              $0.225 \pm 0.437$ &            $0.008 \pm 0.01$ &                                  $0.502 \pm 0.005$ \\
  imfcc &    $\mathbf{0.919 \pm 0.001}$ &              $0.311 \pm 0.454$ &           $0.023 \pm 0.043$ &                                   $0.511 \pm 0.02$ \\
  lfcc  &             $0.916 \pm 0.014$ &     $\mathbf{0.494 \pm 0.395}$ &           $0.076 \pm 0.044$ &                                  $0.533 \pm 0.023$ \\
  mfcc  &             $0.912 \pm 0.006$ &              $0.228 \pm 0.212$ &           $0.098 \pm 0.091$ &                                  $0.541 \pm 0.039$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_dkitchen_snr_10db_to_dkitchen_snr_10db_model_dkitchen_snr_10db_dkitchen_snr_10db/test_dkitchen_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping dkitchen snr 10db to dkitchen snr 10db model dkitchen snr 10db dkitchen snr 10db test dkitchen snr 10db}
  \label{tab:equal_mapping_dkitchen_snr_10db_to_dkitchen_snr_10db_model_dkitchen_snr_10db_dkitchen_snr_10db_test_dkitchen_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.923 \pm 0.009$ &              $0.586 \pm 0.122$ &            $0.329 \pm 0.08$ &                                  $0.652 \pm 0.032$ \\
  igfcc &             $0.921 \pm 0.007$ &              $0.489 \pm 0.327$ &           $0.137 \pm 0.082$ &                                  $0.563 \pm 0.038$ \\
  imfcc &              $0.91 \pm 0.014$ &              $0.435 \pm 0.186$ &           $0.147 \pm 0.045$ &                                  $0.562 \pm 0.013$ \\
  lfcc  &    $\mathbf{0.929 \pm 0.007}$ &              $0.609 \pm 0.097$ &  $\mathbf{0.427 \pm 0.054}$ &                           $\mathbf{0.7 \pm 0.022}$ \\
  mfcc  &    $\mathbf{0.929 \pm 0.012}$ &     $\mathbf{0.623 \pm 0.156}$ &            $0.41 \pm 0.054$ &                                  $0.692 \pm 0.023$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_dkitchen_snr_15db_to_dkitchen_snr_15db_model_dkitchen_snr_15db_dkitchen_snr_15db/test_dkitchen_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping dkitchen snr 15db to dkitchen snr 15db model dkitchen snr 15db dkitchen snr 15db test dkitchen snr 15db}
  \label{tab:equal_mapping_dkitchen_snr_15db_to_dkitchen_snr_15db_model_dkitchen_snr_15db_dkitchen_snr_15db_test_dkitchen_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.94 \pm 0.009$ &              $0.692 \pm 0.109$ &           $0.497 \pm 0.085$ &                                   $0.738 \pm 0.04$ \\
  igfcc &             $0.908 \pm 0.015$ &              $0.444 \pm 0.083$ &           $0.348 \pm 0.081$ &                                  $0.653 \pm 0.032$ \\
  imfcc &             $0.917 \pm 0.011$ &              $0.547 \pm 0.212$ &           $0.325 \pm 0.066$ &                                  $0.647 \pm 0.025$ \\
  lfcc  &             $0.946 \pm 0.003$ &              $0.683 \pm 0.031$ &  $\mathbf{0.642 \pm 0.075}$ &                         $\mathbf{0.808 \pm 0.035}$ \\
  mfcc  &    $\mathbf{0.949 \pm 0.007}$ &     $\mathbf{0.738 \pm 0.107}$ &           $0.619 \pm 0.105$ &                                  $0.799 \pm 0.048$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_dkitchen_snr_20db_to_dkitchen_snr_20db_model_dkitchen_snr_20db_dkitchen_snr_20db/test_dkitchen_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping dkitchen snr 20db to dkitchen snr 20db model dkitchen snr 20db dkitchen snr 20db test dkitchen snr 20db}
  \label{tab:equal_mapping_dkitchen_snr_20db_to_dkitchen_snr_20db_model_dkitchen_snr_20db_dkitchen_snr_20db_test_dkitchen_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.958 \pm 0.01$ &              $0.788 \pm 0.083$ &           $0.681 \pm 0.112$ &                                  $0.832 \pm 0.055$ \\
  igfcc &             $0.936 \pm 0.017$ &               $0.61 \pm 0.108$ &           $0.651 \pm 0.103$ &                                   $0.806 \pm 0.05$ \\
  imfcc &             $0.949 \pm 0.006$ &               $0.731 \pm 0.07$ &           $0.603 \pm 0.068$ &                                  $0.791 \pm 0.032$ \\
  lfcc  &             $0.968 \pm 0.003$ &              $0.837 \pm 0.067$ &  $\mathbf{0.766 \pm 0.077}$ &                         $\mathbf{0.876 \pm 0.035}$ \\
  mfcc  &    $\mathbf{0.969 \pm 0.004}$ &     $\mathbf{0.871 \pm 0.042}$ &           $0.725 \pm 0.027$ &                                  $0.858 \pm 0.013$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_dkitchen_snr_5db_to_dkitchen_snr_5db_model_dkitchen_snr_5db_dkitchen_snr_5db/test_dkitchen_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping dkitchen snr 5db to dkitchen snr 5db model dkitchen snr 5db dkitchen snr 5db test dkitchen snr 5db}
  \label{tab:equal_mapping_dkitchen_snr_5db_to_dkitchen_snr_5db_model_dkitchen_snr_5db_dkitchen_snr_5db_test_dkitchen_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.914 \pm 0.004$ &              $0.445 \pm 0.049$ &           $0.207 \pm 0.041$ &                                  $0.592 \pm 0.018$ \\
  igfcc &             $0.906 \pm 0.011$ &              $0.255 \pm 0.164$ &           $0.121 \pm 0.074$ &                                   $0.548 \pm 0.03$ \\
  imfcc &             $0.912 \pm 0.006$ &              $0.368 \pm 0.112$ &           $0.087 \pm 0.049$ &                                  $0.536 \pm 0.022$ \\
  lfcc  &    $\mathbf{0.922 \pm 0.003}$ &     $\mathbf{0.556 \pm 0.057}$ &             $0.2 \pm 0.014$ &                                  $0.593 \pm 0.007$ \\
  mfcc  &             $0.919 \pm 0.002$ &                $0.5 \pm 0.028$ &  $\mathbf{0.219 \pm 0.036}$ &                           $\mathbf{0.6 \pm 0.017}$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_pcafeter_snr_0db_to_pcafeter_snr_0db_model_pcafeter_snr_0db_pcafeter_snr_0db/test_pcafeter_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping pcafeter snr 0db to pcafeter snr 0db model pcafeter snr 0db pcafeter snr 0db test pcafeter snr 0db}
  \label{tab:equal_mapping_pcafeter_snr_0db_to_pcafeter_snr_0db_model_pcafeter_snr_0db_pcafeter_snr_0db_test_pcafeter_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &    $\mathbf{0.908 \pm 0.023}$ &              $0.106 \pm 0.174$ &            $0.03 \pm 0.048$ &                                  $0.508 \pm 0.011$ \\
  igfcc &             $0.907 \pm 0.023$ &              $0.175 \pm 0.205$ &           $0.043 \pm 0.075$ &                                  $0.513 \pm 0.022$ \\
  imfcc &    $\mathbf{0.908 \pm 0.011}$ &     $\mathbf{0.392 \pm 0.371}$ &  $\mathbf{0.122 \pm 0.108}$ &                          $\mathbf{0.55 \pm 0.045}$ \\
  lfcc  &             $0.906 \pm 0.016$ &              $0.177 \pm 0.175$ &           $0.086 \pm 0.094$ &                                  $0.532 \pm 0.035$ \\
  mfcc  &             $0.891 \pm 0.035$ &               $0.116 \pm 0.12$ &           $0.083 \pm 0.089$ &                                  $0.523 \pm 0.027$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_pcafeter_snr_10db_to_pcafeter_snr_10db_model_pcafeter_snr_10db_pcafeter_snr_10db/test_pcafeter_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping pcafeter snr 10db to pcafeter snr 10db model pcafeter snr 10db pcafeter snr 10db test pcafeter snr 10db}
  \label{tab:equal_mapping_pcafeter_snr_10db_to_pcafeter_snr_10db_model_pcafeter_snr_10db_pcafeter_snr_10db_test_pcafeter_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.897 \pm 0.027$ &              $0.473 \pm 0.313$ &           $0.231 \pm 0.122$ &                                  $0.593 \pm 0.052$ \\
  igfcc &             $0.904 \pm 0.016$ &              $0.441 \pm 0.067$ &  $\mathbf{0.533 \pm 0.053}$ &                         $\mathbf{0.735 \pm 0.019}$ \\
  imfcc &             $0.884 \pm 0.019$ &              $0.355 \pm 0.063$ &           $0.491 \pm 0.038$ &                                  $0.705 \pm 0.025$ \\
  lfcc  &    $\mathbf{0.915 \pm 0.016}$ &     $\mathbf{0.504 \pm 0.104}$ &           $0.465 \pm 0.104$ &                                    $0.71 \pm 0.04$ \\
  mfcc  &             $0.903 \pm 0.008$ &               $0.36 \pm 0.061$ &            $0.25 \pm 0.091$ &                                   $0.605 \pm 0.04$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_pcafeter_snr_15db_to_pcafeter_snr_15db_model_pcafeter_snr_15db_pcafeter_snr_15db/test_pcafeter_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping pcafeter snr 15db to pcafeter snr 15db model pcafeter snr 15db pcafeter snr 15db test pcafeter snr 15db}
  \label{tab:equal_mapping_pcafeter_snr_15db_to_pcafeter_snr_15db_model_pcafeter_snr_15db_pcafeter_snr_15db_test_pcafeter_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.921 \pm 0.013$ &              $0.554 \pm 0.102$ &           $0.353 \pm 0.097$ &                                  $0.662 \pm 0.041$ \\
  igfcc &             $0.932 \pm 0.008$ &              $0.565 \pm 0.039$ &  $\mathbf{0.706 \pm 0.084}$ &                          $\mathbf{0.829 \pm 0.04}$ \\
  imfcc &             $0.924 \pm 0.013$ &               $0.536 \pm 0.07$ &           $0.668 \pm 0.038$ &                                  $0.808 \pm 0.015$ \\
  lfcc  &    $\mathbf{0.946 \pm 0.007}$ &      $\mathbf{0.686 \pm 0.08}$ &           $0.637 \pm 0.054$ &                                  $0.805 \pm 0.023$ \\
  mfcc  &              $0.932 \pm 0.01$ &              $0.627 \pm 0.118$ &           $0.467 \pm 0.049$ &                                   $0.72 \pm 0.021$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_pcafeter_snr_20db_to_pcafeter_snr_20db_model_pcafeter_snr_20db_pcafeter_snr_20db/test_pcafeter_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping pcafeter snr 20db to pcafeter snr 20db model pcafeter snr 20db pcafeter snr 20db test pcafeter snr 20db}
  \label{tab:equal_mapping_pcafeter_snr_20db_to_pcafeter_snr_20db_model_pcafeter_snr_20db_pcafeter_snr_20db_test_pcafeter_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.946 \pm 0.014$ &              $0.683 \pm 0.114$ &           $0.661 \pm 0.034$ &                                   $0.816 \pm 0.02$ \\
  igfcc &             $0.956 \pm 0.015$ &              $0.699 \pm 0.096$ &  $\mathbf{0.834 \pm 0.038}$ &                           $\mathbf{0.9 \pm 0.019}$ \\
  imfcc &             $0.954 \pm 0.015$ &              $0.696 \pm 0.099$ &           $0.808 \pm 0.048$ &                                  $0.888 \pm 0.025$ \\
  lfcc  &    $\mathbf{0.966 \pm 0.005}$ &     $\mathbf{0.833 \pm 0.092}$ &           $0.747 \pm 0.046$ &                                  $0.866 \pm 0.019$ \\
  mfcc  &             $0.953 \pm 0.008$ &              $0.762 \pm 0.126$ &           $0.649 \pm 0.059$ &                                  $0.814 \pm 0.023$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_pcafeter_snr_5db_to_pcafeter_snr_5db_model_pcafeter_snr_5db_pcafeter_snr_5db/test_pcafeter_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping pcafeter snr 5db to pcafeter snr 5db model pcafeter snr 5db pcafeter snr 5db test pcafeter snr 5db}
  \label{tab:equal_mapping_pcafeter_snr_5db_to_pcafeter_snr_5db_model_pcafeter_snr_5db_pcafeter_snr_5db_test_pcafeter_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.905 \pm 0.021$ &               $0.24 \pm 0.311$ &           $0.062 \pm 0.064$ &                                  $0.521 \pm 0.022$ \\
  igfcc &              $0.896 \pm 0.03$ &              $0.322 \pm 0.274$ &             $0.19 \pm 0.15$ &                                  $0.574 \pm 0.053$ \\
  imfcc &    $\mathbf{0.906 \pm 0.006}$ &     $\mathbf{0.379 \pm 0.047}$ &  $\mathbf{0.252 \pm 0.121}$ &                         $\mathbf{0.608 \pm 0.053}$ \\
  lfcc  &             $0.895 \pm 0.018$ &              $0.233 \pm 0.146$ &           $0.207 \pm 0.152$ &                                  $0.581 \pm 0.065$ \\
  mfcc  &             $0.891 \pm 0.029$ &              $0.201 \pm 0.152$ &           $0.118 \pm 0.077$ &                                  $0.539 \pm 0.025$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_spsquare_snr_0db_to_spsquare_snr_0db_model_spsquare_snr_0db_spsquare_snr_0db/test_spsquare_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping spsquare snr 0db to spsquare snr 0db model spsquare snr 0db spsquare snr 0db test spsquare snr 0db}
  \label{tab:equal_mapping_spsquare_snr_0db_to_spsquare_snr_0db_model_spsquare_snr_0db_spsquare_snr_0db_test_spsquare_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.885 \pm 0.055$ &              $0.035 \pm 0.077$ &           $0.086 \pm 0.193$ &                                  $0.521 \pm 0.059$ \\
  igfcc &    $\mathbf{0.905 \pm 0.019}$ &              $0.344 \pm 0.202$ &  $\mathbf{0.417 \pm 0.241}$ &                         $\mathbf{0.682 \pm 0.104}$ \\
  imfcc &             $0.904 \pm 0.023$ &     $\mathbf{0.406 \pm 0.299}$ &            $0.34 \pm 0.274$ &                                  $0.647 \pm 0.115$ \\
  lfcc  &             $0.883 \pm 0.033$ &              $0.253 \pm 0.154$ &           $0.342 \pm 0.222$ &                                   $0.637 \pm 0.09$ \\
  mfcc  &             $0.885 \pm 0.032$ &              $0.112 \pm 0.137$ &           $0.125 \pm 0.156$ &                                  $0.539 \pm 0.066$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_spsquare_snr_10db_to_spsquare_snr_10db_model_spsquare_snr_10db_spsquare_snr_10db/test_spsquare_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping spsquare snr 10db to spsquare snr 10db model spsquare snr 10db spsquare snr 10db test spsquare snr 10db}
  \label{tab:equal_mapping_spsquare_snr_10db_to_spsquare_snr_10db_model_spsquare_snr_10db_spsquare_snr_10db_test_spsquare_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.91 \pm 0.019$ &               $0.47 \pm 0.084$ &           $0.587 \pm 0.101$ &                                  $0.763 \pm 0.044$ \\
  igfcc &              $0.957 \pm 0.01$ &              $0.698 \pm 0.073$ &   $\mathbf{0.845 \pm 0.02}$ &                                  $0.906 \pm 0.008$ \\
  imfcc &    $\mathbf{0.964 \pm 0.008}$ &      $\mathbf{0.752 \pm 0.07}$ &  $\mathbf{0.845 \pm 0.044}$ &                           $\mathbf{0.91 \pm 0.02}$ \\
  lfcc  &             $0.951 \pm 0.014$ &               $0.68 \pm 0.094$ &           $0.789 \pm 0.038$ &                                   $0.877 \pm 0.02$ \\
  mfcc  &             $0.918 \pm 0.024$ &              $0.548 \pm 0.135$ &            $0.51 \pm 0.111$ &                                   $0.732 \pm 0.04$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_spsquare_snr_15db_to_spsquare_snr_15db_model_spsquare_snr_15db_spsquare_snr_15db/test_spsquare_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping spsquare snr 15db to spsquare snr 15db model spsquare snr 15db spsquare snr 15db test spsquare snr 15db}
  \label{tab:equal_mapping_spsquare_snr_15db_to_spsquare_snr_15db_model_spsquare_snr_15db_spsquare_snr_15db_test_spsquare_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.948 \pm 0.007$ &               $0.679 \pm 0.04$ &           $0.692 \pm 0.087$ &                                  $0.831 \pm 0.042$ \\
  igfcc &     $\mathbf{0.98 \pm 0.005}$ &     $\mathbf{0.867 \pm 0.071}$ &           $0.906 \pm 0.035$ &                         $\mathbf{0.946 \pm 0.014}$ \\
  imfcc &             $0.978 \pm 0.005$ &              $0.864 \pm 0.093$ &           $0.883 \pm 0.063$ &                                  $0.935 \pm 0.026$ \\
  lfcc  &             $0.976 \pm 0.004$ &              $0.814 \pm 0.023$ &  $\mathbf{0.909 \pm 0.031}$ &                                  $0.945 \pm 0.016$ \\
  mfcc  &              $0.958 \pm 0.01$ &              $0.763 \pm 0.115$ &           $0.744 \pm 0.053$ &                                   $0.861 \pm 0.02$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_spsquare_snr_20db_to_spsquare_snr_20db_model_spsquare_snr_20db_spsquare_snr_20db/test_spsquare_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping spsquare snr 20db to spsquare snr 20db model spsquare snr 20db spsquare snr 20db test spsquare snr 20db}
  \label{tab:equal_mapping_spsquare_snr_20db_to_spsquare_snr_20db_model_spsquare_snr_20db_spsquare_snr_20db_test_spsquare_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.965 \pm 0.006$ &              $0.828 \pm 0.052$ &           $0.718 \pm 0.046$ &                                  $0.852 \pm 0.023$ \\
  igfcc &             $0.985 \pm 0.006$ &              $0.879 \pm 0.055$ &  $\mathbf{0.951 \pm 0.017}$ &                                   $0.969 \pm 0.01$ \\
  imfcc &    $\mathbf{0.989 \pm 0.004}$ &       $\mathbf{0.92 \pm 0.03}$ &           $0.947 \pm 0.042$ &                          $\mathbf{0.97 \pm 0.021}$ \\
  lfcc  &             $0.985 \pm 0.003$ &              $0.874 \pm 0.042$ &  $\mathbf{0.951 \pm 0.022}$ &                                  $0.969 \pm 0.009$ \\
  mfcc  &             $0.977 \pm 0.004$ &              $0.843 \pm 0.059$ &           $0.883 \pm 0.049$ &                                  $0.934 \pm 0.022$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_spsquare_snr_5db_to_spsquare_snr_5db_model_spsquare_snr_5db_spsquare_snr_5db/test_spsquare_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping spsquare snr 5db to spsquare snr 5db model spsquare snr 5db spsquare snr 5db test spsquare snr 5db}
  \label{tab:equal_mapping_spsquare_snr_5db_to_spsquare_snr_5db_model_spsquare_snr_5db_spsquare_snr_5db_test_spsquare_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.878 \pm 0.047$ &              $0.258 \pm 0.176$ &           $0.282 \pm 0.213$ &                                  $0.607 \pm 0.079$ \\
  igfcc &    $\mathbf{0.934 \pm 0.009}$ &     $\mathbf{0.578 \pm 0.052}$ &   $\mathbf{0.735 \pm 0.06}$ &                         $\mathbf{0.843 \pm 0.023}$ \\
  imfcc &              $0.926 \pm 0.01$ &              $0.539 \pm 0.048$ &            $0.732 \pm 0.03$ &                                  $0.838 \pm 0.009$ \\
  lfcc  &              $0.914 \pm 0.01$ &               $0.48 \pm 0.051$ &           $0.629 \pm 0.104$ &                                   $0.784 \pm 0.05$ \\
  mfcc  &              $0.874 \pm 0.03$ &              $0.217 \pm 0.122$ &           $0.328 \pm 0.217$ &                                  $0.625 \pm 0.083$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_ssn_morten_snr_0db_to_ssn_morten_snr_0db_model_ssn_morten_snr_0db_ssn_morten_snr_0db/test_ssn_morten_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping ssn morten snr 0db to ssn morten snr 0db model ssn morten snr 0db ssn morten snr 0db test ssn morten snr 0db}
  \label{tab:equal_mapping_ssn_morten_snr_0db_to_ssn_morten_snr_0db_model_ssn_morten_snr_0db_ssn_morten_snr_0db_test_ssn_morten_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.91 \pm 0.014$ &              $0.098 \pm 0.148$ &           $0.023 \pm 0.043$ &                                  $0.506 \pm 0.012$ \\
  igfcc &     $\mathbf{0.93 \pm 0.013}$ &     $\mathbf{0.595 \pm 0.116}$ &  $\mathbf{0.528 \pm 0.042}$ &                         $\mathbf{0.747 \pm 0.018}$ \\
  imfcc &             $0.919 \pm 0.007$ &              $0.241 \pm 0.363$ &             $0.073 \pm 0.1$ &                                  $0.533 \pm 0.045$ \\
  lfcc  &             $0.918 \pm 0.005$ &              $0.412 \pm 0.253$ &           $0.113 \pm 0.066$ &                                   $0.551 \pm 0.03$ \\
  mfcc  &              $0.91 \pm 0.018$ &               $0.266 \pm 0.31$ &           $0.098 \pm 0.094$ &                                   $0.54 \pm 0.037$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_ssn_morten_snr_10db_to_ssn_morten_snr_10db_model_ssn_morten_snr_10db_ssn_morten_snr_10db/test_ssn_morten_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping ssn morten snr 10db to ssn morten snr 10db model ssn morten snr 10db ssn morten snr 10db test ssn morten snr 10db}
  \label{tab:equal_mapping_ssn_morten_snr_10db_to_ssn_morten_snr_10db_model_ssn_morten_snr_10db_ssn_morten_snr_10db_test_ssn_morten_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.908 \pm 0.011$ &              $0.191 \pm 0.178$ &           $0.114 \pm 0.117$ &                                  $0.546 \pm 0.049$ \\
  igfcc &    $\mathbf{0.968 \pm 0.007}$ &      $\mathbf{0.77 \pm 0.069}$ &  $\mathbf{0.876 \pm 0.038}$ &                         $\mathbf{0.926 \pm 0.015}$ \\
  imfcc &             $0.928 \pm 0.014$ &              $0.714 \pm 0.248$ &           $0.335 \pm 0.094$ &                                  $0.658 \pm 0.038$ \\
  lfcc  &             $0.901 \pm 0.012$ &              $0.403 \pm 0.055$ &           $0.439 \pm 0.112$ &                                    $0.69 \pm 0.05$ \\
  mfcc  &             $0.902 \pm 0.019$ &              $0.394 \pm 0.134$ &           $0.222 \pm 0.087$ &                                  $0.592 \pm 0.034$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_ssn_morten_snr_15db_to_ssn_morten_snr_15db_model_ssn_morten_snr_15db_ssn_morten_snr_15db/test_ssn_morten_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping ssn morten snr 15db to ssn morten snr 15db model ssn morten snr 15db ssn morten snr 15db test ssn morten snr 15db}
  \label{tab:equal_mapping_ssn_morten_snr_15db_to_ssn_morten_snr_15db_model_ssn_morten_snr_15db_ssn_morten_snr_15db_test_ssn_morten_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.909 \pm 0.012$ &               $0.445 \pm 0.06$ &            $0.43 \pm 0.034$ &                                  $0.691 \pm 0.016$ \\
  igfcc &    $\mathbf{0.979 \pm 0.002}$ &     $\mathbf{0.843 \pm 0.021}$ &   $\mathbf{0.909 \pm 0.01}$ &                         $\mathbf{0.947 \pm 0.003}$ \\
  imfcc &              $0.96 \pm 0.006$ &              $0.756 \pm 0.058$ &           $0.758 \pm 0.057$ &                                  $0.868 \pm 0.027$ \\
  lfcc  &             $0.939 \pm 0.005$ &              $0.622 \pm 0.036$ &           $0.639 \pm 0.082$ &                                  $0.802 \pm 0.037$ \\
  mfcc  &              $0.92 \pm 0.017$ &               $0.54 \pm 0.128$ &           $0.503 \pm 0.089$ &                                   $0.73 \pm 0.037$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_ssn_morten_snr_20db_to_ssn_morten_snr_20db_model_ssn_morten_snr_20db_ssn_morten_snr_20db/test_ssn_morten_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping ssn morten snr 20db to ssn morten snr 20db model ssn morten snr 20db ssn morten snr 20db test ssn morten snr 20db}
  \label{tab:equal_mapping_ssn_morten_snr_20db_to_ssn_morten_snr_20db_model_ssn_morten_snr_20db_ssn_morten_snr_20db_test_ssn_morten_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.938 \pm 0.011$ &              $0.652 \pm 0.117$ &           $0.541 \pm 0.075$ &                                  $0.757 \pm 0.035$ \\
  igfcc &    $\mathbf{0.988 \pm 0.002}$ &     $\mathbf{0.909 \pm 0.015}$ &  $\mathbf{0.944 \pm 0.012}$ &                         $\mathbf{0.968 \pm 0.006}$ \\
  imfcc &              $0.98 \pm 0.006$ &              $0.869 \pm 0.063$ &           $0.887 \pm 0.024$ &                                  $0.937 \pm 0.011$ \\
  lfcc  &             $0.964 \pm 0.007$ &              $0.754 \pm 0.085$ &           $0.842 \pm 0.058$ &                                  $0.908 \pm 0.024$ \\
  mfcc  &             $0.954 \pm 0.009$ &              $0.746 \pm 0.071$ &           $0.669 \pm 0.091$ &                                  $0.824 \pm 0.045$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_ssn_morten_snr_5db_to_ssn_morten_snr_5db_model_ssn_morten_snr_5db_ssn_morten_snr_5db/test_ssn_morten_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping ssn morten snr 5db to ssn morten snr 5db model ssn morten snr 5db ssn morten snr 5db test ssn morten snr 5db}
  \label{tab:equal_mapping_ssn_morten_snr_5db_to_ssn_morten_snr_5db_model_ssn_morten_snr_5db_ssn_morten_snr_5db_test_ssn_morten_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.914 \pm 0.01$ &              $0.176 \pm 0.266$ &           $0.045 \pm 0.073$ &                                  $0.518 \pm 0.029$ \\
  igfcc &     $\mathbf{0.948 \pm 0.01}$ &     $\mathbf{0.669 \pm 0.084}$ &    $\mathbf{0.76 \pm 0.08}$ &                         $\mathbf{0.862 \pm 0.033}$ \\
  imfcc &             $0.921 \pm 0.009$ &               $0.607 \pm 0.23$ &           $0.242 \pm 0.058$ &                                  $0.611 \pm 0.023$ \\
  lfcc  &             $0.907 \pm 0.012$ &              $0.341 \pm 0.135$ &           $0.105 \pm 0.041$ &                                  $0.541 \pm 0.017$ \\
  mfcc  &             $0.912 \pm 0.013$ &              $0.342 \pm 0.239$ &           $0.125 \pm 0.072$ &                                  $0.554 \pm 0.032$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_tbus_snr_0db_to_tbus_snr_0db_model_tbus_snr_0db_tbus_snr_0db/test_tbus_snr_0db/table.tex <==
\begin{table}
  \caption{equal mapping tbus snr 0db to tbus snr 0db model tbus snr 0db tbus snr 0db test tbus snr 0db}
  \label{tab:equal_mapping_tbus_snr_0db_to_tbus_snr_0db_model_tbus_snr_0db_tbus_snr_0db_test_tbus_snr_0db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &               $0.91 \pm 0.02$ &              $0.466 \pm 0.117$ &           $0.438 \pm 0.093$ &                                  $0.695 \pm 0.046$ \\
  igfcc &    $\mathbf{0.952 \pm 0.008}$ &      $\mathbf{0.745 \pm 0.09}$ &  $\mathbf{0.654 \pm 0.096}$ &                         $\mathbf{0.816 \pm 0.045}$ \\
  imfcc &              $0.95 \pm 0.006$ &              $0.732 \pm 0.098$ &           $0.637 \pm 0.088$ &                                  $0.807 \pm 0.038$ \\
  lfcc  &             $0.945 \pm 0.011$ &               $0.691 \pm 0.08$ &           $0.592 \pm 0.089$ &                                  $0.784 \pm 0.045$ \\
  mfcc  &             $0.937 \pm 0.011$ &               $0.67 \pm 0.138$ &           $0.557 \pm 0.104$ &                                  $0.764 \pm 0.042$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_tbus_snr_10db_to_tbus_snr_10db_model_tbus_snr_10db_tbus_snr_10db/test_tbus_snr_10db/table.tex <==
\begin{table}
  \caption{equal mapping tbus snr 10db to tbus snr 10db model tbus snr 10db tbus snr 10db test tbus snr 10db}
  \label{tab:equal_mapping_tbus_snr_10db_to_tbus_snr_10db_model_tbus_snr_10db_tbus_snr_10db_test_tbus_snr_10db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.966 \pm 0.006$ &              $0.818 \pm 0.052$ &           $0.747 \pm 0.037$ &                                  $0.866 \pm 0.019$ \\
  igfcc &             $0.984 \pm 0.006$ &              $0.874 \pm 0.059$ &            $0.94 \pm 0.025$ &                                  $0.964 \pm 0.012$ \\
  imfcc &    $\mathbf{0.991 \pm 0.004}$ &     $\mathbf{0.928 \pm 0.033}$ &  $\mathbf{0.966 \pm 0.021}$ &                          $\mathbf{0.98 \pm 0.012}$ \\
  lfcc  &             $0.983 \pm 0.005$ &              $0.886 \pm 0.058$ &           $0.917 \pm 0.023$ &                                  $0.953 \pm 0.011$ \\
  mfcc  &             $0.974 \pm 0.003$ &               $0.833 \pm 0.03$ &           $0.849 \pm 0.053$ &                                  $0.917 \pm 0.025$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_tbus_snr_15db_to_tbus_snr_15db_model_tbus_snr_15db_tbus_snr_15db/test_tbus_snr_15db/table.tex <==
\begin{table}
  \caption{equal mapping tbus snr 15db to tbus snr 15db model tbus snr 15db tbus snr 15db test tbus snr 15db}
  \label{tab:equal_mapping_tbus_snr_15db_to_tbus_snr_15db_model_tbus_snr_15db_tbus_snr_15db_test_tbus_snr_15db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.975 \pm 0.003$ &              $0.835 \pm 0.044$ &            $0.86 \pm 0.035$ &                                  $0.922 \pm 0.016$ \\
  igfcc &             $0.991 \pm 0.002$ &               $0.941 \pm 0.03$ &           $0.951 \pm 0.016$ &                                  $0.973 \pm 0.007$ \\
  imfcc &    $\mathbf{0.993 \pm 0.003}$ &     $\mathbf{0.945 \pm 0.021}$ &  $\mathbf{0.973 \pm 0.026}$ &                         $\mathbf{0.984 \pm 0.013}$ \\
  lfcc  &             $0.988 \pm 0.004$ &              $0.907 \pm 0.024$ &           $0.955 \pm 0.026$ &                                  $0.973 \pm 0.014$ \\
  mfcc  &             $0.983 \pm 0.001$ &              $0.886 \pm 0.022$ &            $0.91 \pm 0.015$ &                                   $0.95 \pm 0.007$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_tbus_snr_20db_to_tbus_snr_20db_model_tbus_snr_20db_tbus_snr_20db/test_tbus_snr_20db/table.tex <==
\begin{table}
  \caption{equal mapping tbus snr 20db to tbus snr 20db model tbus snr 20db tbus snr 20db test tbus snr 20db}
  \label{tab:equal_mapping_tbus_snr_20db_to_tbus_snr_20db_model_tbus_snr_20db_tbus_snr_20db_test_tbus_snr_20db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &              $0.98 \pm 0.006$ &               $0.895 \pm 0.04$ &            $0.86 \pm 0.043$ &                                  $0.926 \pm 0.023$ \\
  igfcc &             $0.995 \pm 0.002$ &              $0.967 \pm 0.023$ &  $\mathbf{0.977 \pm 0.016}$ &                         $\mathbf{0.987 \pm 0.008}$ \\
  imfcc &    $\mathbf{0.997 \pm 0.003}$ &      $\mathbf{0.992 \pm 0.01}$ &           $0.974 \pm 0.031$ &                                  $0.986 \pm 0.016$ \\
  lfcc  &              $0.99 \pm 0.005$ &              $0.932 \pm 0.045$ &           $0.954 \pm 0.041$ &                                   $0.974 \pm 0.02$ \\
  mfcc  &             $0.985 \pm 0.002$ &              $0.936 \pm 0.026$ &           $0.872 \pm 0.028$ &                                  $0.933 \pm 0.013$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/equal_mapping_tbus_snr_5db_to_tbus_snr_5db_model_tbus_snr_5db_tbus_snr_5db/test_tbus_snr_5db/table.tex <==
\begin{table}
  \caption{equal mapping tbus snr 5db to tbus snr 5db model tbus snr 5db tbus snr 5db test tbus snr 5db}
  \label{tab:equal_mapping_tbus_snr_5db_to_tbus_snr_5db_model_tbus_snr_5db_tbus_snr_5db_test_tbus_snr_5db}
  \centering
  \begin{tabular}{lllll}
  \toprule
  {} & \rotatebox{0}{test\_accuracy} & \rotatebox{0}{test\_precision} & \rotatebox{0}{test\_recall} & \rotatebox{0}{test\_receiver\_operator\_characteristic\_auc} \\
  index &                               &                                &                             &                                                              \\
  \midrule
  gfcc  &             $0.948 \pm 0.002$ &              $0.702 \pm 0.026$ &            $0.62 \pm 0.034$ &                                  $0.798 \pm 0.016$ \\
  igfcc &    $\mathbf{0.978 \pm 0.003}$ &     $\mathbf{0.859 \pm 0.036}$ &           $0.868 \pm 0.042$ &                          $\mathbf{0.928 \pm 0.02}$ \\
  imfcc &             $0.975 \pm 0.005$ &              $0.833 \pm 0.042$ &  $\mathbf{0.872 \pm 0.033}$ &                         $\mathbf{0.928 \pm 0.016}$ \\
  lfcc  &             $0.971 \pm 0.003$ &              $0.812 \pm 0.045$ &           $0.837 \pm 0.059$ &                                   $0.91 \pm 0.027$ \\
  mfcc  &             $0.964 \pm 0.007$ &              $0.822 \pm 0.117$ &            $0.747 \pm 0.12$ &                                  $0.865 \pm 0.054$ \\
  \bottomrule
  \end{tabular}
\end{table}

==> figures/latex/1618499599/table.tex <==
\begin{tabular}{lllllll}
\toprule
                          & transformation & \rotatebox{0}{gfcc} & \rotatebox{0}{igfcc} & \rotatebox{0}{imfcc} & \rotatebox{0}{lfcc} & \rotatebox{0}{mfcc} \\
\midrule
equal\_mapping\_bbl\_morten\_snr\_0db\_to\_bbl\_morten\_snr\_0db\_model\_bbl\_morten\_snr\_0db\_bbl\_morten\_snr\_0db & test\_bbl\_morten\_snr\_0db &   $0.528 \pm 0.029$ &    $0.687 \pm 0.059$ &    $0.654 \pm 0.027$ &   $0.573 \pm 0.046$ &   $0.533 \pm 0.047$ \\
equal\_mapping\_bbl\_morten\_snr\_10db\_to\_bbl\_morten\_snr\_10db\_model\_bbl\_morten\_snr\_10db\_bbl\_morten\_snr\_10db & test\_bbl\_morten\_snr\_10db &    $0.668 \pm 0.04$ &    $0.901 \pm 0.011$ &    $0.878 \pm 0.016$ &     $0.78 \pm 0.02$ &   $0.706 \pm 0.038$ \\
equal\_mapping\_bbl\_morten\_snr\_15db\_to\_bbl\_morten\_snr\_15db\_model\_bbl\_morten\_snr\_15db\_bbl\_morten\_snr\_15db & test\_bbl\_morten\_snr\_15db &   $0.742 \pm 0.025$ &    $0.951 \pm 0.015$ &    $0.921 \pm 0.024$ &   $0.857 \pm 0.012$ &   $0.798 \pm 0.017$ \\
equal\_mapping\_bbl\_morten\_snr\_20db\_to\_bbl\_morten\_snr\_20db\_model\_bbl\_morten\_snr\_20db\_bbl\_morten\_snr\_20db & test\_bbl\_morten\_snr\_20db &   $0.838 \pm 0.033$ &    $0.955 \pm 0.009$ &    $0.953 \pm 0.009$ &   $0.901 \pm 0.022$ &    $0.867 \pm 0.03$ \\
equal\_mapping\_bbl\_morten\_snr\_5db\_to\_bbl\_morten\_snr\_5db\_model\_bbl\_morten\_snr\_5db\_bbl\_morten\_snr\_5db & test\_bbl\_morten\_snr\_5db &    $0.576 \pm 0.02$ &    $0.806 \pm 0.048$ &    $0.793 \pm 0.032$ &   $0.702 \pm 0.022$ &   $0.621 \pm 0.042$ \\
equal\_mapping\_dkitchen\_snr\_0db\_to\_dkitchen\_snr\_0db\_model\_dkitchen\_snr\_0db\_dkitchen\_snr\_0db & test\_dkitchen\_snr\_0db &   $0.562 \pm 0.023$ &    $0.502 \pm 0.005$ &     $0.511 \pm 0.02$ &   $0.533 \pm 0.023$ &   $0.541 \pm 0.039$ \\
equal\_mapping\_dkitchen\_snr\_10db\_to\_dkitchen\_snr\_10db\_model\_dkitchen\_snr\_10db\_dkitchen\_snr\_10db & test\_dkitchen\_snr\_10db &   $0.652 \pm 0.032$ &    $0.563 \pm 0.038$ &    $0.562 \pm 0.013$ &     $0.7 \pm 0.022$ &   $0.692 \pm 0.023$ \\
equal\_mapping\_dkitchen\_snr\_15db\_to\_dkitchen\_snr\_15db\_model\_dkitchen\_snr\_15db\_dkitchen\_snr\_15db & test\_dkitchen\_snr\_15db &    $0.738 \pm 0.04$ &    $0.653 \pm 0.032$ &    $0.647 \pm 0.025$ &   $0.808 \pm 0.035$ &   $0.799 \pm 0.048$ \\
equal\_mapping\_dkitchen\_snr\_20db\_to\_dkitchen\_snr\_20db\_model\_dkitchen\_snr\_20db\_dkitchen\_snr\_20db & test\_dkitchen\_snr\_20db &   $0.832 \pm 0.055$ &     $0.806 \pm 0.05$ &    $0.791 \pm 0.032$ &   $0.876 \pm 0.035$ &   $0.858 \pm 0.013$ \\
equal\_mapping\_dkitchen\_snr\_5db\_to\_dkitchen\_snr\_5db\_model\_dkitchen\_snr\_5db\_dkitchen\_snr\_5db & test\_dkitchen\_snr\_5db &   $0.592 \pm 0.018$ &     $0.548 \pm 0.03$ &    $0.536 \pm 0.022$ &   $0.593 \pm 0.007$ &     $0.6 \pm 0.017$ \\
equal\_mapping\_pcafeter\_snr\_0db\_to\_pcafeter\_snr\_0db\_model\_pcafeter\_snr\_0db\_pcafeter\_snr\_0db & test\_pcafeter\_snr\_0db &   $0.508 \pm 0.011$ &    $0.513 \pm 0.022$ &     $0.55 \pm 0.045$ &   $0.532 \pm 0.035$ &   $0.523 \pm 0.027$ \\
equal\_mapping\_pcafeter\_snr\_10db\_to\_pcafeter\_snr\_10db\_model\_pcafeter\_snr\_10db\_pcafeter\_snr\_10db & test\_pcafeter\_snr\_10db &   $0.593 \pm 0.052$ &    $0.735 \pm 0.019$ &    $0.705 \pm 0.025$ &     $0.71 \pm 0.04$ &    $0.605 \pm 0.04$ \\
equal\_mapping\_pcafeter\_snr\_15db\_to\_pcafeter\_snr\_15db\_model\_pcafeter\_snr\_15db\_pcafeter\_snr\_15db & test\_pcafeter\_snr\_15db &   $0.662 \pm 0.041$ &     $0.829 \pm 0.04$ &    $0.808 \pm 0.015$ &   $0.805 \pm 0.023$ &    $0.72 \pm 0.021$ \\
equal\_mapping\_pcafeter\_snr\_20db\_to\_pcafeter\_snr\_20db\_model\_pcafeter\_snr\_20db\_pcafeter\_snr\_20db & test\_pcafeter\_snr\_20db &    $0.816 \pm 0.02$ &      $0.9 \pm 0.019$ &    $0.888 \pm 0.025$ &   $0.866 \pm 0.019$ &   $0.814 \pm 0.023$ \\
equal\_mapping\_pcafeter\_snr\_5db\_to\_pcafeter\_snr\_5db\_model\_pcafeter\_snr\_5db\_pcafeter\_snr\_5db & test\_pcafeter\_snr\_5db &   $0.521 \pm 0.022$ &    $0.574 \pm 0.053$ &    $0.608 \pm 0.053$ &   $0.581 \pm 0.065$ &   $0.539 \pm 0.025$ \\
equal\_mapping\_spsquare\_snr\_0db\_to\_spsquare\_snr\_0db\_model\_spsquare\_snr\_0db\_spsquare\_snr\_0db & test\_spsquare\_snr\_0db &   $0.521 \pm 0.059$ &    $0.682 \pm 0.104$ &    $0.647 \pm 0.115$ &    $0.637 \pm 0.09$ &   $0.539 \pm 0.066$ \\
equal\_mapping\_spsquare\_snr\_10db\_to\_spsquare\_snr\_10db\_model\_spsquare\_snr\_10db\_spsquare\_snr\_10db & test\_spsquare\_snr\_10db &   $0.763 \pm 0.044$ &    $0.906 \pm 0.008$ &      $0.91 \pm 0.02$ &    $0.877 \pm 0.02$ &    $0.732 \pm 0.04$ \\
equal\_mapping\_spsquare\_snr\_15db\_to\_spsquare\_snr\_15db\_model\_spsquare\_snr\_15db\_spsquare\_snr\_15db & test\_spsquare\_snr\_15db &   $0.831 \pm 0.042$ &    $0.946 \pm 0.014$ &    $0.935 \pm 0.026$ &   $0.945 \pm 0.016$ &    $0.861 \pm 0.02$ \\
equal\_mapping\_spsquare\_snr\_20db\_to\_spsquare\_snr\_20db\_model\_spsquare\_snr\_20db\_spsquare\_snr\_20db & test\_spsquare\_snr\_20db &   $0.852 \pm 0.023$ &     $0.969 \pm 0.01$ &     $0.97 \pm 0.021$ &   $0.969 \pm 0.009$ &   $0.934 \pm 0.022$ \\
equal\_mapping\_spsquare\_snr\_5db\_to\_spsquare\_snr\_5db\_model\_spsquare\_snr\_5db\_spsquare\_snr\_5db & test\_spsquare\_snr\_5db &   $0.607 \pm 0.079$ &    $0.843 \pm 0.023$ &    $0.838 \pm 0.009$ &    $0.784 \pm 0.05$ &   $0.625 \pm 0.083$ \\
equal\_mapping\_ssn\_morten\_snr\_0db\_to\_ssn\_morten\_snr\_0db\_model\_ssn\_morten\_snr\_0db\_ssn\_morten\_snr\_0db & test\_ssn\_morten\_snr\_0db &   $0.506 \pm 0.012$ &    $0.747 \pm 0.018$ &    $0.533 \pm 0.045$ &    $0.551 \pm 0.03$ &    $0.54 \pm 0.037$ \\
equal\_mapping\_ssn\_morten\_snr\_10db\_to\_ssn\_morten\_snr\_10db\_model\_ssn\_morten\_snr\_10db\_ssn\_morten\_snr\_10db & test\_ssn\_morten\_snr\_10db &   $0.546 \pm 0.049$ &    $0.926 \pm 0.015$ &    $0.658 \pm 0.038$ &     $0.69 \pm 0.05$ &   $0.592 \pm 0.034$ \\
equal\_mapping\_ssn\_morten\_snr\_15db\_to\_ssn\_morten\_snr\_15db\_model\_ssn\_morten\_snr\_15db\_ssn\_morten\_snr\_15db & test\_ssn\_morten\_snr\_15db &   $0.691 \pm 0.016$ &    $0.947 \pm 0.003$ &    $0.868 \pm 0.027$ &   $0.802 \pm 0.037$ &    $0.73 \pm 0.037$ \\
equal\_mapping\_ssn\_morten\_snr\_20db\_to\_ssn\_morten\_snr\_20db\_model\_ssn\_morten\_snr\_20db\_ssn\_morten\_snr\_20db & test\_ssn\_morten\_snr\_20db &   $0.757 \pm 0.035$ &    $0.968 \pm 0.006$ &    $0.937 \pm 0.011$ &   $0.908 \pm 0.024$ &   $0.824 \pm 0.045$ \\
equal\_mapping\_ssn\_morten\_snr\_5db\_to\_ssn\_morten\_snr\_5db\_model\_ssn\_morten\_snr\_5db\_ssn\_morten\_snr\_5db & test\_ssn\_morten\_snr\_5db &   $0.518 \pm 0.029$ &    $0.862 \pm 0.033$ &    $0.611 \pm 0.023$ &   $0.541 \pm 0.017$ &   $0.554 \pm 0.032$ \\
equal\_mapping\_tbus\_snr\_0db\_to\_tbus\_snr\_0db\_model\_tbus\_snr\_0db\_tbus\_snr\_0db & test\_tbus\_snr\_0db &   $0.695 \pm 0.046$ &    $0.816 \pm 0.045$ &    $0.807 \pm 0.038$ &   $0.784 \pm 0.045$ &   $0.764 \pm 0.042$ \\
equal\_mapping\_tbus\_snr\_10db\_to\_tbus\_snr\_10db\_model\_tbus\_snr\_10db\_tbus\_snr\_10db & test\_tbus\_snr\_10db &   $0.866 \pm 0.019$ &    $0.964 \pm 0.012$ &     $0.98 \pm 0.012$ &   $0.953 \pm 0.011$ &   $0.917 \pm 0.025$ \\
equal\_mapping\_tbus\_snr\_15db\_to\_tbus\_snr\_15db\_model\_tbus\_snr\_15db\_tbus\_snr\_15db & test\_tbus\_snr\_15db &   $0.922 \pm 0.016$ &    $0.973 \pm 0.007$ &    $0.984 \pm 0.013$ &   $0.973 \pm 0.014$ &    $0.95 \pm 0.007$ \\
equal\_mapping\_tbus\_snr\_20db\_to\_tbus\_snr\_20db\_model\_tbus\_snr\_20db\_tbus\_snr\_20db & test\_tbus\_snr\_20db &   $0.926 \pm 0.023$ &    $0.987 \pm 0.008$ &    $0.986 \pm 0.016$ &    $0.974 \pm 0.02$ &   $0.933 \pm 0.013$ \\
equal\_mapping\_tbus\_snr\_5db\_to\_tbus\_snr\_5db\_model\_tbus\_snr\_5db\_tbus\_snr\_5db & test\_tbus\_snr\_5db &   $0.798 \pm 0.016$ &     $0.928 \pm 0.02$ &    $0.928 \pm 0.016$ &    $0.91 \pm 0.027$ &   $0.865 \pm 0.054$ \\
merge\_ab\_test\_ab\_model\_ab\_ab & test\_a &   $0.942 \pm 0.007$ &    $0.985 \pm 0.002$ &    $0.989 \pm 0.002$ &   $0.976 \pm 0.001$ &   $0.964 \pm 0.002$ \\
                          & test\_a\_b &   $0.948 \pm 0.006$ &    $0.986 \pm 0.001$ &    $0.989 \pm 0.002$ &   $0.979 \pm 0.001$ &   $0.966 \pm 0.001$ \\
                          & test\_b &   $0.972 \pm 0.012$ &     $0.99 \pm 0.005$ &     $0.99 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.974 \pm 0.004$ \\
noises\_all\_snr\_to\_pcafeter\_model\_all\_noise\_snr\_all\_noise\_snr & test\_pcafeter\_snr\_0db &   $0.579 \pm 0.024$ &    $0.644 \pm 0.017$ &    $0.651 \pm 0.017$ &    $0.634 \pm 0.03$ &   $0.585 \pm 0.019$ \\
                          & test\_pcafeter\_snr\_0db\_pcafeter\_snr\_5db\_pcafeter\_snr\_10db\_pcafeter\_snr\_15db\_pcafeter\_snr\_20db &   $0.695 \pm 0.019$ &    $0.805 \pm 0.009$ &    $0.801 \pm 0.016$ &   $0.771 \pm 0.016$ &   $0.711 \pm 0.026$ \\
                          & test\_pcafeter\_snr\_10db &   $0.689 \pm 0.031$ &    $0.818 \pm 0.016$ &    $0.805 \pm 0.032$ &   $0.785 \pm 0.027$ &   $0.707 \pm 0.033$ \\
                          & test\_pcafeter\_snr\_15db &    $0.76 \pm 0.022$ &    $0.898 \pm 0.017$ &    $0.887 \pm 0.022$ &   $0.844 \pm 0.011$ &   $0.784 \pm 0.041$ \\
                          & test\_pcafeter\_snr\_20db &   $0.814 \pm 0.032$ &    $0.939 \pm 0.007$ &     $0.93 \pm 0.017$ &    $0.89 \pm 0.017$ &   $0.851 \pm 0.022$ \\
                          & test\_pcafeter\_snr\_5db &   $0.634 \pm 0.023$ &    $0.726 \pm 0.018$ &    $0.731 \pm 0.027$ &   $0.701 \pm 0.014$ &   $0.627 \pm 0.023$ \\
truncated\_a\_model\_a\_a & test\_a &    $0.915 \pm 0.02$ &    $0.981 \pm 0.003$ &     $0.98 \pm 0.003$ &   $0.961 \pm 0.003$ &   $0.941 \pm 0.013$ \\
                          & test\_b &    $0.694 \pm 0.04$ &    $0.932 \pm 0.012$ &     $0.946 \pm 0.01$ &   $0.692 \pm 0.127$ &   $0.576 \pm 0.072$ \\
truncated\_a\_silence\_model\_silence\_silence & test\_silence &   $0.965 \pm 0.014$ &    $0.995 \pm 0.004$ &    $0.993 \pm 0.006$ &   $0.988 \pm 0.006$ &    $0.97 \pm 0.016$ \\
                          & test\_speech &   $0.661 \pm 0.058$ &    $0.851 \pm 0.071$ &     $0.823 \pm 0.06$ &   $0.746 \pm 0.042$ &   $0.724 \pm 0.074$ \\
truncated\_a\_speech\_model\_speech\_speech & test\_silence &   $0.863 \pm 0.033$ &    $0.988 \pm 0.011$ &    $0.987 \pm 0.009$ &    $0.948 \pm 0.02$ &   $0.937 \pm 0.017$ \\
                          & test\_speech &   $0.679 \pm 0.036$ &    $0.945 \pm 0.018$ &    $0.944 \pm 0.021$ &   $0.886 \pm 0.028$ &   $0.833 \pm 0.051$ \\
truncated\_b\_model\_b\_b & test\_a &   $0.528 \pm 0.011$ &    $0.676 \pm 0.034$ &    $0.672 \pm 0.091$ &   $0.625 \pm 0.057$ &   $0.527 \pm 0.015$ \\
                          & test\_b &   $0.982 \pm 0.004$ &    $0.991 \pm 0.005$ &    $0.991 \pm 0.007$ &   $0.988 \pm 0.003$ &   $0.983 \pm 0.005$ \\
\bottomrule
\end{tabular}


==> figures/latex/auc_tables.tex <==


% \begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
% \input{figures/latex/1614926381/table}
% \end{adjustbox}

% \begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
% \input{figures/latex/1618398903/table}
% \end{adjustbox}

% \begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
% \input{figures/latex/1618499599/table}
% \end{adjustbox}



==> figures/latex/bloated_tables.tex <==

\textcolor{red}{Massive number of tables, we should probably choose a few interesting ones, some redundancy here. I will combine the results across experiment test set for each model for brevity. But you can have a look to confirm results.}

\paragraph{model ab}

\input{figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_a_b/table}
\input{figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_a/table}
\input{figures/latex/1614926381/merge_ab_test_ab_model_ab_ab/test_b/table}

\paragraph{model a}

\input{figures/latex/1614926381/truncated_a_model_a_a/test_a/table}
\input{figures/latex/1614926381/truncated_a_model_a_a/test_b/table}

\paragraph{model b}

\input{figures/latex/1614926381/truncated_b_model_b_b/test_a/table}
\input{figures/latex/1614926381/truncated_b_model_b_b/test_b/table}

\paragraph{model speech}

\input{figures/latex/1614926381/truncated_a_speech_model_speech_speech/test_silence/table}
\input{figures/latex/1614926381/truncated_a_speech_model_speech_speech/test_speech/table}

\paragraph{model silence}

\input{figures/latex/1614926381/truncated_a_silence_model_silence_silence/test_silence/table}
\input{figures/latex/1614926381/truncated_a_silence_model_silence_silence/test_speech/table}


\paragraph{model all noise to cafeteria}


\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_0db/table}
\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_5db/table}
\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_10db/table}
\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_15db/table}
\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_20db/table}

\input{figures/latex/1618398903/noises_all_snr_to_pcafeter_model_all_noise_snr_all_noise_snr/test_pcafeter_snr_0db_pcafeter_snr_5db_pcafeter_snr_10db_pcafeter_snr_15db_pcafeter_snr_20db/table}


\paragraph{model bus}


\input{figures/latex/1618499599/equal_mapping_tbus_snr_0db_to_tbus_snr_0db_model_tbus_snr_0db_tbus_snr_0db/test_tbus_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_tbus_snr_5db_to_tbus_snr_5db_model_tbus_snr_5db_tbus_snr_5db/test_tbus_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_tbus_snr_10db_to_tbus_snr_10db_model_tbus_snr_10db_tbus_snr_10db/test_tbus_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_tbus_snr_15db_to_tbus_snr_15db_model_tbus_snr_15db_tbus_snr_15db/test_tbus_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_tbus_snr_20db_to_tbus_snr_20db_model_tbus_snr_20db_tbus_snr_20db/test_tbus_snr_20db/table}


\paragraph{model square}


\input{figures/latex/1618499599/equal_mapping_spsquare_snr_0db_to_spsquare_snr_0db_model_spsquare_snr_0db_spsquare_snr_0db/test_spsquare_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_spsquare_snr_5db_to_spsquare_snr_5db_model_spsquare_snr_5db_spsquare_snr_5db/test_spsquare_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_spsquare_snr_10db_to_spsquare_snr_10db_model_spsquare_snr_10db_spsquare_snr_10db/test_spsquare_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_spsquare_snr_15db_to_spsquare_snr_15db_model_spsquare_snr_15db_spsquare_snr_15db/test_spsquare_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_spsquare_snr_20db_to_spsquare_snr_20db_model_spsquare_snr_20db_spsquare_snr_20db/test_spsquare_snr_20db/table}


\paragraph{model cafeteria}


\input{figures/latex/1618499599/equal_mapping_pcafeter_snr_0db_to_pcafeter_snr_0db_model_pcafeter_snr_0db_pcafeter_snr_0db/test_pcafeter_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_pcafeter_snr_5db_to_pcafeter_snr_5db_model_pcafeter_snr_5db_pcafeter_snr_5db/test_pcafeter_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_pcafeter_snr_10db_to_pcafeter_snr_10db_model_pcafeter_snr_10db_pcafeter_snr_10db/test_pcafeter_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_pcafeter_snr_15db_to_pcafeter_snr_15db_model_pcafeter_snr_15db_pcafeter_snr_15db/test_pcafeter_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_pcafeter_snr_20db_to_pcafeter_snr_20db_model_pcafeter_snr_20db_pcafeter_snr_20db/test_pcafeter_snr_20db/table}

\paragraph{model kitchen}


\input{figures/latex/1618499599/equal_mapping_dkitchen_snr_0db_to_dkitchen_snr_0db_model_dkitchen_snr_0db_dkitchen_snr_0db/test_dkitchen_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_dkitchen_snr_5db_to_dkitchen_snr_5db_model_dkitchen_snr_5db_dkitchen_snr_5db/test_dkitchen_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_dkitchen_snr_10db_to_dkitchen_snr_10db_model_dkitchen_snr_10db_dkitchen_snr_10db/test_dkitchen_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_dkitchen_snr_15db_to_dkitchen_snr_15db_model_dkitchen_snr_15db_dkitchen_snr_15db/test_dkitchen_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_dkitchen_snr_20db_to_dkitchen_snr_20db_model_dkitchen_snr_20db_dkitchen_snr_20db/test_dkitchen_snr_20db/table}



\paragraph{model babble}


\input{figures/latex/1618499599/equal_mapping_bbl_morten_snr_0db_to_bbl_morten_snr_0db_model_bbl_morten_snr_0db_bbl_morten_snr_0db/test_bbl_morten_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_bbl_morten_snr_5db_to_bbl_morten_snr_5db_model_bbl_morten_snr_5db_bbl_morten_snr_5db/test_bbl_morten_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_bbl_morten_snr_10db_to_bbl_morten_snr_10db_model_bbl_morten_snr_10db_bbl_morten_snr_10db/test_bbl_morten_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_bbl_morten_snr_15db_to_bbl_morten_snr_15db_model_bbl_morten_snr_15db_bbl_morten_snr_15db/test_bbl_morten_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_bbl_morten_snr_20db_to_bbl_morten_snr_20db_model_bbl_morten_snr_20db_bbl_morten_snr_20db/test_bbl_morten_snr_20db/table}

\paragraph{model speech shaped noise}


\input{figures/latex/1618499599/equal_mapping_ssn_morten_snr_0db_to_ssn_morten_snr_0db_model_ssn_morten_snr_0db_ssn_morten_snr_0db/test_ssn_morten_snr_0db/table}

\input{figures/latex/1618499599/equal_mapping_ssn_morten_snr_5db_to_ssn_morten_snr_5db_model_ssn_morten_snr_5db_ssn_morten_snr_5db/test_ssn_morten_snr_5db/table}

\input{figures/latex/1618499599/equal_mapping_ssn_morten_snr_10db_to_ssn_morten_snr_10db_model_ssn_morten_snr_10db_ssn_morten_snr_10db/test_ssn_morten_snr_10db/table}

\input{figures/latex/1618499599/equal_mapping_ssn_morten_snr_15db_to_ssn_morten_snr_15db_model_ssn_morten_snr_15db_ssn_morten_snr_15db/test_ssn_morten_snr_15db/table}

\input{figures/latex/1618499599/equal_mapping_ssn_morten_snr_20db_to_ssn_morten_snr_20db_model_ssn_morten_snr_20db_ssn_morten_snr_20db/test_ssn_morten_snr_20db/table}





==> tables/speech_silence.tex <==
\begin{table*}[hb]
\centering
\caption{Mean and standard deviation of ROCAUC for speech and non-speech data sets. \textit{speech \& ns} denotes both speech and non-speech attack datasets.}
\label{tab:rocauc_speechsilence_old}
\medskip
\begin{adjustbox}{width=12cm, center=\tablewidth}
\begin{tabular}{lccccc}
\toprule
\aefdbcrowx{filter bank}                       [GFCC]              [IGFCC]                     [IMFCC]                     [LFCC]             [MFCC]
\aefdbcrowx{train set \hspace{0.5cm} test set}
\midrule                          
\aefdbcrowx{non-speech}
\aefdbcrowx{\hspace{1.5cm} non-speech}       [$.965 \pm .014$] [$\mathbf{.995 \pm .004}$][$.993 \pm .006$]         [$.988 \pm .006$][ $.97 \pm .016$]
\aefdbcrowx{\hspace{1.5cm} speech}        [$.661 \pm .058$] [$\mathbf{.851 \pm .071}$][ $.823 \pm .06$]         [$.746 \pm .042$][$.724 \pm .074$]
\aefdbcrowx{speech }
\aefdbcrowx{\hspace{1.5cm} speech}        [$.679 \pm .036$] [$\mathbf{.945 \pm .018}$][$.944 \pm .021$]         [$.886 \pm .028$][$.833 \pm .051$]
\aefdbcrowx{\hspace{1.5cm} non-speech}       [$.863 \pm .033$] [$\mathbf{.988 \pm .011}$][$.987 \pm .009$]         [ $.948 \pm .02$][$.937 \pm .017$] 
\aefdbcrowx{speech \& ns}
\aefdbcrowx{\hspace{1.5cm} s\&ns} [$.894 \pm .006$] [$.978 \pm .005$]         [$\mathbf{.982 \pm .008}$][$.941 \pm .013$][$.929 \pm .013$]
\aefdbcrowx{\hspace{1.5cm} non-speech}       [$.973 \pm .01$]  [$.997 \pm .001$]         [$\mathbf{.999 \pm .002}$][ $.98 \pm .016$][$.986 \pm .002$]
\aefdbcrowx{\hspace{1.5cm} speech}        [$.858 \pm .008$] [ $.97 \pm .007$]         [$\mathbf{.975 \pm .011}$][$.925 \pm .015$][$.903 \pm .019$]
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/white_black_box.tex <==
\begin{table*}[hbt!]
\centering
\caption{Mean and standard deviation of ROCAUC for white-box and black-box data sets. \textit{w\&b} denotes both white-box and black-box attacks.}
\label{tab:rocauc_ab_old}
\medskip
\begin{adjustbox}{width=12cm, center=\tablewidth}
\begin{tabular}{lccccc}
\toprule
\aefdbcrowx{filter bank}                           [GFCC]             [IGFCC]                      [IMFCC]                     [LFCC]              [MFCC]
\aefdbcrowx{train set \hspace{0.5cm} test set}
\midrule
\aefdbcrowx{white-box}
\aefdbcrowx{\hspace{1.5cm} white-box}         [$.915 \pm .02$ ][$\mathbf{.981 \pm .003}$] [$.98 \pm .003$]          [$.961 \pm .003$][$.941 \pm .013$]
\aefdbcrowx{\hspace{1.5cm} black-box}         [$.694 \pm .04$ ][$.932 \pm .012$]          [$\mathbf{.946 \pm .01}$] [$.692 \pm .127$][$.576 \pm .072$]  
\aefdbcrowx{black-box}
\aefdbcrowx{\hspace{1.5cm} white-box}         [$.528 \pm .011$][$.676 \pm .034$]          [$\mathbf{.672 \pm .091}$][$.625 \pm .057$][$.527 \pm .015$] 
\aefdbcrowx{\hspace{1.5cm} black-box}         [$.982 \pm .004$][$\mathbf{.991 \pm .005}$] [$.991 \pm .007$]         [$.988 \pm .003$][$.983 \pm .005$]            
\aefdbcrowx{w\&b-box}
\aefdbcrowx{\hspace{1.5cm} w\&b-box}   [$.948 \pm .006$][$.986 \pm .001$]          [$\mathbf{.989 \pm .002}$][$.979 \pm .001$][$.966 \pm .001$]
\aefdbcrowx{\hspace{1.5cm} white-box}         [$.942 \pm .007$][$.985 \pm .002$]          [$\mathbf{.989 \pm .002}$][$.976 \pm .001$][$.964 \pm .002$]
\aefdbcrowx{\hspace{1.5cm} black-box}         [$.972 \pm .012$][$\mathbf{.99 \pm .005}$]  [$.99 \pm .007$]          [$.988 \pm .003$][$.974 \pm .004$]
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> utilities/color_table.tex <==
\pgfplotsset{compat=1.17}

\pgfplotstableset{
    /color cells/min/.initial=0,
    /color cells/max/.initial=1000,
    /color cells/textcolor/.initial=,
    color cells/.code={%% Usage: 'color cells={min=<value which is mapped to lowest color>, max = <value which is mapped to largest>}
        \pgfqkeys{/color cells}{#1}%
        \pgfkeysalso{%
            postproc cell content/.code={%
                %
                \begingroup
	                %
	                \pgfkeysgetvalue{/pgfplots/table/@preprocessed cell content}\value                 % acquire the value before any number printer changed it:
	                \pgfmathfloatparsenumber{\value}%
	                \pgfmathfloattofixed{\pgfmathresult}%
	                \let\value=\pgfmathresult
	                %
	                \pgfplotscolormapaccess                % map that value:
	                [\pgfkeysvalueof{/color cells/min}:\pgfkeysvalueof{/color cells/max}]
	                {\value}
	                {\pgfkeysvalueof{/pgfplots/colormap name}}
	                % now, \pgfmathresult contains {<R>,<G>,<B>}
	                %
	                \pgfkeysgetvalue{/pgfplots/table/@cell content}\typesetvalue % acquire the value AFTER any preprocessor or typesetter (like number printer) worked on it:
	                %                \pgfkeysgetvalue{/color cells/textcolor}\textcolorvalue
	                \ifdim\value pt<.55pt\relax
	                	\def\textcolorvalue{white}%
	                \else
	               	 \def\textcolorvalue{black}%
	                \fi
	                %
	                \toks0=\expandafter{\typesetvalue}% % tex-expansion control see http://tex.stackexchange.com/questions/12668/where-do-i-start-latex-programming/27589#27589
	                \xdef\temp{%
	                    \noexpand\pgfkeysalso{%
	                        @cell content={%
	                            \noexpand\cellcolor[rgb]{\pgfmathresult}%
	                            \noexpand\definecolor{mapped color}{rgb}{\pgfmathresult}%
	                            \ifx\textcolorvalue\empty
	                            \else
	                            \noexpand\color{\textcolorvalue}%
	                            \fi
	                            \the\toks0 %
	                        }%
	                    }%
	                }%
                \endgroup
                \temp
            }%
        }%
    }
}

\newcommand{\printconfusionmatrix}[1][]{
\pgfplotstableread[
    col sep=comma,
    string type,
    header=true,
%every head row/.style={before row=\toprule,after row=\midrule},
%every last row/.style={after row=\bottomrule},
%display columns/angle/.style={string type,postproc cell content/.code={\ang{#1}}},
%display columns/magnitude/.style={column name={$a$}},
]{#1}{\mytable}

\pgfplotstablegetrowsof{\mytable}
\pgfmathsetmacro{\startColNo}{0}
\pgfmathsetmacro{\startRowNo}{1}
\pgfmathsetmacro\lastRowNo{\pgfplotsretval}
\pgfplotstablegetcolsof{\mytable}
\pgfmathsetmacro\lastColNo{\pgfplotsretval-1}

\pgfplotsinvokeforeach{\startColNo,...,\lastColNo} {%   Specify head row
	\pgfplotstableset{
	        columns/#1/.style = {column name=#1},
	    }
	}%
	\pgfplotstableset{% Create new column
	    create on use/newcol/.style={ create col/set list={\startRowNo,...,\lastRowNo}},
	    columns/newcol/.style={column name={}, postproc cell content/.style={@cell content=##1} 
   	 }%
}%

	 \pgfplotstabletypeset[
	        color cells={min=0.0,max=1.0,textcolor=-mapped color!80!black},
	        /pgfplots/colormap/blackwhite,
	        set decimal separator={,},
	        columns={newcol,0,1,...,\lastColNo},
	        column type=r,   %string type,
	    ]{\mytable}
}

==> utilities/underscore_replacement.tex <==
\newcommand{\filename}[1]{\emph{\replunderscores{#1}}}
\newcommand{\reprname}[1]{\replaceunderscore{#1}} % TODO: General replace with argument

\makeatletter % \expandafter for the case that the filename is given in a command
\newcommand{\replunderscores}[1]
{\expandafter\@repl@underscores#1_\relax}
\def\@repl@underscores#1_#2\relax{%
    \ifx \relax #2\relax            % #2 is empty => finish
        #1%
    \else                           % #2 is not empty => underscore was contained, needs to be replaced
        #1%
        \textunderscore             % continue replacing
        \@repl@underscores#2\relax  % #2 ends with an extra underscore so I don't need to add another one
    \fi
}
\makeatother


\makeatletter % \expandafter for the case that the filename is given in a command
\newcommand{\replaceunderscore}[1]
{\expandafter\@repl@underscores#1_\relax}
\def\@repl@underscores#1_#2\relax{%
    \ifx \relax #2\relax            % #2 is empty => finish
        #1%
    \else                           % #2 is not empty => underscore was contained, needs to be replaced
        #1%
        \              % continue replacing
        \@repl@underscores#2\relax  % #2 ends with an extra underscore so I don't need to add another one
    \fi
}
\makeatother

